NeuFENet: Neural Finite Element Solutions with Theoretical Bounds for Parametric PDEs

We consider a mesh-based approach for training a neural network to produce field predictions of solutions to parametric partial differential equations (PDEs). This approach contrasts current approaches for "neural PDE solvers" that employ collocation-based methods to make point-wise predictions of solutions to PDEs. This approach has the advantage of naturally enforcing different boundary conditions as well as ease of invoking well-developed PDE theory -- including analysis of numerical stability and convergence -- to obtain capacity bounds for our proposed neural networks in discretized domains. We explore our mesh-based strategy, called NeuFENet, using a weighted Galerkin loss function based on the Finite Element Method (FEM) on a parametric elliptic PDE. The weighted Galerkin loss (FEM loss) is similar to an energy functional that produces improved solutions, satisfies a priori mesh convergence, and can model Dirichlet and Neumann boundary conditions. We prove theoretically, and illustrate with experiments, convergence results analogous to mesh convergence analysis deployed in finite element solutions to PDEs. These results suggest that a mesh-based neural network approach serves as a promising approach for solving parametric PDEs with theoretical bounds.

==> arxiv-pack-2/cmdDefs.tex <==
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% New Commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\theoremstyle{plain}
\newtheorem{definition}{Definition}[section]
% \theoremstyle{remark}
% \newtheorem*{remark}{\textbf{Remark}}

\newtheorem{theorem}{\textbf{Theorem}}[section]
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[theorem]{\textbf{Lemma}}
\newtheorem{assumption}[theorem]{\textbf{Assumption}}
\newtheorem{claim}{\textbf{Claim}}
\newtheorem{note}{\textbf{Note}}
\theoremstyle{remark}
\newtheorem{remark}{\textbf{Remark}}
%\newtheorem{corollary}{\textbf{Corollary}}
\renewcommand\qedsymbol{$\blacksquare$}

\newcommand{\bunderline}[2][4]{\underline{#2\mkern-#1mu}\mkern#1mu}
\newcommand{\doubleunderline}[1]{\underline{\underline{#1}}}

\newcommand{\etal}{\textit{et al.}}

\newcommand{\spatialD}{D}
\newcommand{\temporalInterval}{I_T}
\newcommand{\ith}{i^{th}}
\newcommand{\xcomp}[1]{x_{#1}}
\newcommand{\xii}{\xcomp{i}}
\newcommand{\ucomp}[1]{u_{#1}}
\newcommand{\ui}{\ucomp{i}}
\newcommand{\fcomp}[1]{f_{#1}}
\newcommand{\fii}{\fcomp{i}}
\newcommand{\xvec}{\mvec{x}}
\newcommand{\uc}[1]{u^c_{#1}}
\newcommand{\uf}[1]{u^f_{#1}}
\newcommand{\uvec}{\mvec{u}}
\newcommand{\vvec}{\mvec{v}}
\newcommand{\wvec}{\mvec{w}}
\newcommand{\uvech}{\mvec{u}^h}
\newcommand{\vvech}{\mvec{v}^h}
\newcommand{\wvech}{\mvec{w}^h}
\newcommand{\ph}{p^h}
\newcommand{\qh}{q^h}
\newcommand{\resUvec}{\mvec{r}(\uvec)}
\newcommand{\resUvech}{\mvec{r}(\uvech)}
\newcommand{\resUi}{r(\ui)}
\newcommand{\resP}{r(p)}
\newcommand{\partialder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\timeder}[1]{\partialder{#1}{t}}
\newcommand{\taum}{\tau_m}
\newcommand{\tauc}{\tau_c}
\newcommand{\diffusivity}{\nu}
\newcommand{\stochdiff}{\tilde{\nu}}
\newcommand{\visco}{\nu}
\newcommand{\pder}[1]{\partialder{p}{\xii}}

\newcommand{\Na}{N_a}
\newcommand{\Nb}{N_b}

\newcommand{\nel}{n_{el}}
\newcommand{\uh}{u^h}
\newcommand{\vh}{v^h}
\newcommand{\wh}{w^h}
\newcommand{\er}{e}
\newcommand{\eh}{e^h}
\newcommand{\ei}{\hat{e}}
\newcommand{\spaceV}{V}
\newcommand{\spaceVh}{V^h}
\newcommand{\spaceVtheta}{V_\netparams}
\newcommand{\spaceVhtheta}{V^h_\netparams}
\newcommand{\interpolant}{\mathcal{I}^h}
\newcommand{\interp}[1]{\interpolant #1}
\newcommand{\nsd}{n}
\newcommand{\adv}{\mvec{a}}
\newcommand{\advcomp}[1]{a_{#1}}
\newcommand{\bit}{\Gamma_{_0}}
\newcommand{\bft}{\Gamma_{_T}}
\newcommand{\mesh}{\mathcal{K}^h}
\newcommand{\edgeset}{\mathcal{E}_h}
\newcommand{\grad}{\mvec{{\nabla}}}
\newcommand{\gradsym}{\mvec{{\nabla^s}}}
\newcommand{\gradst}{\tilde{{\mvec{{\nabla}}}}}
\newcommand{\laplacian}{\Delta}
\newcommand{\ellipticA}{A}
\newcommand{\ellipticAmat}{\mmat{\ellipticA}}
\newcommand{\ellipticB}{B}
\newcommand{\ellipticBvec}{\mmat{\ellipticB}}
\newcommand{\ellipticC}{\tilde{\mvec{C}}}
\newcommand{\ellipticD}{\tilde{\mvec{D}}}
\newcommand{\ellipticI}{\tilde{\mvec{I}}}
\newcommand{\bform}{b}
\newcommand{\bformh}{\bform^h}
\newcommand{\lform}{l}
\newcommand{\lformh}{\lform^h}
\newcommand{\glspar}{\epsilon}

\newcommand{\ustar}{u_{*}}
\newcommand{\uNeural}{u_{\netparams}}
\newcommand{\uneuralOpt}{u_{\netparamsExact}}
\newcommand{\uneuralDiscOmega}{u^h_{N_s}}
\newcommand{\uneuralPerfOmega}{\uh}

\newcommand{\uExact}{u}
\newcommand{\uNeuralExactOpt}{u_{\netparamsExact}}
\newcommand{\uDiscrete}{\uh}

%\newcommand{\eGen}{\mathcal{E}_G}
%\newcommand{\eOpt}{\mathcal{E}_{\netparams}}
%\newcommand{\eCap}{\mathcal{E}_{\mathcal{H}}}
%\newcommand{\eDis}{\mathcal{E}_h}

\newcommand{\eGen}{e_G}
\newcommand{\eOpt}{e_{\netparams}}
\newcommand{\eCap}{e_{\mathcal{H}}}
\newcommand{\eDis}{e_h}
\newcommand{\errJ}{\mathcal{E}_J}
\newcommand{\errL}{\mathcal{E}_{\hat{L}}}

\newcommand{\mvec}[1]{{\mathbf{#1}}}
\newcommand{\mmat}[1]{{\mathbf{#1}}}
\newcommand{\mat}[1]{\smash{\doubleunderline{#1}}}

\newcommand{\intTimeSpace}{\int_0^T\int_{\spatialD}}
\newcommand{\intSpaceTime}{\int_{\spatialD}\int_0^T}
\newcommand{\intOmega}{\int_{\Omega}}

\newcommand{\setbuilder}[1]{\left\{ #1 \right\}}
\newcommand{\modulus}[1]{| #1 |}
\newcommand{\inner}[2]{\left( #1, #2 \right)}
\newcommand{\innerBig}[2]{\Big( #1, #2 \Big)}
\newcommand{\norm}[1]{\| #1 \|}
\newcommand{\normL}[3][2]{\| #2 \|_{L^{#1}(#3)}}
\newcommand{\normH}[3][1]{\| #2 \|_{H^{#1}(#3)}}
\newcommand{\seminormL}[3][2]{| #2 |_{L^{#1}(#3)}}
\newcommand{\seminormH}[3][1]{| #2 |_{H^{#1}(#3)}}
\newcommand{\normV}[1]{\| #1 \|_{\spaceVh}}
\newcommand{\normVh}[1]{\| #1 \|_{\spaceVh}}
\newcommand{\normVtheta}[1]{\| #1 \|_{\spaceVtheta}}
\newcommand{\normVhtheta}[1]{\| #1 \|_{\spaceVhtheta}}
\newcommand{\normVstar}[1]{\| #1 \|_{\spaceVh,*}}
\newcommand{\normVExpanded}[1]{\frac{1}{2}\normL{#1}{\bft}^2 + 
	\gamma(\normL{\grad(#1)}{\Omega}^2 + \normL{(#1)_t}{\Omega}^2}

\newcommand{\half}{\frac{1}{2}}
\newcommand{\oneOver}[1]{\frac{1}{#1}}
\newcommand{\invCoefOne}{C_{I,1}}
\newcommand{\invCoefTwo}{C_{I,2}}
\newcommand{\approxConstant}{C_{a}}
\newcommand{\traceConstant}{C_{\Gamma}}
\newcommand{\shapeRegularConst}{C_h}

\newcommand{\apriori}{\textit{a priori }}
\newcommand{\aposteriori}{\textit{a posteriori }}

\newcommand{\talyfem}{\textsc{TalyFEM}}
\newcommand{\petsc}{\textsc{PETSc}}
\newcommand{\parmetis}{\textsc{ParMETIS}}
\newcommand{\snes}{\textsc{SNES}}
\newcommand{\ksp}{\textsc{KSP}}

\newcommand{\neuralMap}{G_{nn}}
\newcommand{\netparams}{\theta}
\newcommand{\netparamsExact}{\tilde{\theta}}
\newcommand{\neuralFunction}{u_{nn}}
\newcommand{\neufenet}{\textsc{NeuFENet}}

\newcommand{\N}{\ensuremath{\mathcal{N}}}
\newcommand{\Lop}{\ensuremath{\mathcal{L}}}
% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}
% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}


%%% START MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.
\newcommand{\logLogSlopeTriangle}[5]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1-#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} 
		%%% REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO 
		%%PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in 
		%[xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED 
		%EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to 
		%the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (A)-- node[pos=0.5,anchor=north] {1}
		(B)-- 
		(C)-- node[pos=0.5,anchor=west] {#4}
		cycle;
	}
}
%%% END MACRO FOR ANNOTATION OF TRIANGLE WITH SLOPE %%%.


%%%%%%%%%%%%%%%%%%% Local functions %%%%%%%%%%%%%%%%%%%
%% -- Draw marks
\newbox\dumbox
\newcommand{\mymark}[2]{%
	\setbox\dumbox=\hbox{#2}%
	\hbox to \wd\dumbox{\hss%
		\tikz[overlay,remember picture,baseline=(#1.base)]{ \node (#1) {\box\dumbox}; }%
		\hss}%
}

%% -- Draw small coefficient
\newcommand{\mysmall}[1]{%
	\tikz[overlay,remember picture]{%
		\node[blue,scale=.5, shift={(0,-.1)}] {x#1};%
	}%
}
%%%%%%%%%%%%%%%%%%% Local functions %%%%%%%%%%%%%%%%%%%

\definecolor{cpu3}{HTML}{F44336}
\definecolor{cpu4}{HTML}{2196F3}
\definecolor{cpu1}{HTML}{4CAF50}
\definecolor{cpu2}{HTML}{FFC107}
\definecolor{gpu3}{HTML}{EF9A9A}
\definecolor{gpu4}{HTML}{90CAF9}
\definecolor{gpu1}{HTML}{A5D6A7}
\definecolor{gpu2}{HTML}{FFE082}

\definecolor{cpu5}{HTML}{9932CC}

\newcommand\numRowsK{3}
\newcommand\numColsK{3}
\newcommand{\K}[2]{% #1: row, #2: col
	\edef\Kcol##1##2##3{###2}%
	\edef\Krow##1##2##3{\noexpand\Kcol###1}%
	\Krow
	{1 0 1}
	{0 1 0}
	{1 0 1}%
}

\newcommand{\mynote}[3]{
	\textcolor{#2}{\fbox{\bfseries\sffamily\scriptsize#1}}
	{\small$\blacktriangleright$\textsf{\emph{#3}}$\blacktriangleleft$}
}

\newcommand{\bg}[1]{\mynote{Baskar}{magenta}{#1}}
\newcommand{\ch}[1]{\mynote{Chinmay}{olive}{#1}}
\newcommand{\ab}[1]{\mynote{Aditya}{blue}{#1}}
\newcommand{\bk}[1]{\mynote{Biswajit}{teal}{#1}}

==> arxiv-pack-2/figure_panels/old_pyplot_histograms.tex <==
\begin{figure}[!htb]
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1000.png} 
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1011.png}\\
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1021.png}
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1031.png}\\
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1042.png}
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2122.png}\\
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2133.png}
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2143.png}
\end{figure}

\begin{figure}[!htb]
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line871.png} 
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line890.png}\\
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line910.png}
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2125.png}\\
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2144.png}
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2164.png}\\
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line3445.png}
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line3464.png}
	\caption{XXXXXX}
\end{figure}
\begin{figure}[!htb]
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line3484.png}
	\caption{YYYYYYYYY}
\end{figure}

==> arxiv-pack-2/sections/conclusions.tex <==
\section{Conclusions}
In this paper, we integrate neural PDE methods with numerical methods by performing numerical differentiation (and integration, if needed) instead of using the spatial differentiability. We defined two loss functions (based on FDM and FEM), for obtaining the neural approximate mapping between inputs and the discretized field solution. We demonstrate this framework's performance on poisson equation in 2D, steady heat transfer. We see that the results obtained from the neural PDE approximation (predicted) are match very closely with actual ground truth numerical solution. 


Remark: Pro-Con discussion of this approach versus conventional PINN
\begin{itemize}
    \item Con: From point prediction to field prediction $ => $ larger model
    \item Pro: Leverage rich theory of numerical analysis ..
\end{itemize}

%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=0.85]
%	\newcommand\reclenH{3}
%	\newcommand\reclenV{4}
%	\newcommand\ndiv{4}
%	\newcommand\stepsize{1}
%	\newcommand\xl{0}
%	\newcommand\yl{0}
%	\newcommand\osx{-0.5}
%	\newcommand\osy{0.5}
%	\fill[cpu2] (\xl,\yl) rectangle (\xl+\reclenH,\yl+\reclenV);
%	\draw[step=\stepsize cm] (\xl,\yl) grid (\xl+\reclenH,\yl+\reclenV);
%%	\draw (0, 0) node {$test$};
%	
%	\foreach \y in {0,1,2,3,4}{
%		\draw [fill=red](0,\y) circle (0.1cm);
%		\draw [fill=red](1,\y) circle (0.1cm);
%		\draw [fill=red](2,\y) circle (0.1cm);
%		\draw [fill=red](3,\y) circle (0.1cm);
%	}
%
%	\draw (\osx, 0) node {$e$};
%	\draw (\osx, 1) node {$d$};
%	\draw (\osx, 2) node {$c$};
%	\draw (\osx, 3) node {$b$};
%	\draw (\osx, 4) node {$a$};
%	
%	\draw (0,\reclenV + \osy) node {$1$};
%	\draw (1,\reclenV + \osy) node {$2$};
%	\draw (2,\reclenV + \osy) node {$3$};
%	\draw (3,\reclenV + \osy) node {$4$};
%	\end{tikzpicture}
%	\caption{Test}
%	\label{fig: IBMfig}
%\end{figure}{}

%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=0.85]
%	\fill[cpu1] (0.0,0.0) rectangle (8,8);
%	\fill[cpu1] (0.0,0.0) rectangle (7.5,7.5);
%	 \fill[cpu1] (6.0,0.0) rectangle (7.5,6.0);
%	\fill[cpu2] (0.75,4.5) rectangle (5.25,5.25);
%	\fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
%	\fill[cpu2] (0.75,0.75) rectangle (1.5,4.5);
%	\fill[cpu2] (4.5,0.75) rectangle (5.25,4.5);
%	\fill[cpu2] (0.0,1.5) rectangle (0.75,4.5);
%	\fill[cpu2] (5.25,1.5) rectangle (6.0,4.5);
%	\fill[cpu2] (1.50,0.0) rectangle (4.5,3.0);
%	
%	\fill[cpu4] (4.5,1.5) rectangle (1.5,4.5);
%	\fill[cpu4] (0.75,2.25) rectangle (1.5,3.75);
%	\fill[cpu4] (4.5,2.25) rectangle (5.25,3.75);
%	\fill[cpu4] (2.25,4.5) rectangle (3.75,5.25);
%	\fill[cpu4] (2.25,0.75) rectangle (3.75,1.5);
%	
%	\draw[step=1.5cm, thick] (0,0) grid (7.5,7.5);
%	\draw[-,black, thick] (0,0.75) -- (6,0.75);
%	\draw[-,black, thick] (0,5.25) -- (6,5.25);
%	\draw[-,black, thick] (0.75,0) -- (0.75,6.0);
%	\draw[-,black, thick] (5.25,0) -- (5.25,6.0);
%	\draw[-,black, thick] (2.25,0) -- (2.25,1.5);
%	\draw[-,black, thick] (3.75,0) -- (3.75,1.5);
%	\draw[-,black, thick] (2.25,4.5) -- (2.25,6.0);
%	\draw[-,black, thick] (3.75,4.5) -- (3.75,6.0);
%	
%	\draw[-,black, thick] (0,2.25) -- (1.5,2.25);
%	\draw[-,black, thick] (0,3.75) -- (1.5,3.75);
%	
%	\draw[-,black, thick] (4.5,2.25) -- (6,2.25);
%	\draw[-,black, thick] (4.5,3.75) -- (6,3.75);
%	
%	\draw[red,ultra thick] (3,3 ) circle (2.5cm);
%	
%%	\foreach \x in {0,1.5,...,7.5}{
%%		\draw [fill=red](\x,0.0) circle (0.1cm);
%%		\draw [fill=red](\x,7.5) circle (0.1cm);
%%		\draw [fill=red](\x,6.0) circle (0.1cm);
%%	}
%%	\foreach \y in {0,1.5,...,7.5}{
%%		\draw [fill=red](0.0,\y) circle (0.1cm);
%%		\draw [fill=red](6.0,\y) circle (0.1cm);
%%		\draw [fill=red](7.5,\y) circle (0.1cm);
%%	}
%	
%	\foreach \x in {1.5,3.0,4.5}
%	\foreach \y in {1.5,3.0,4.5}
%	\draw [fill=gray](\x,\y) circle (0.1cm);
%	
%%	\foreach \y in {0.0,0.75,...,5.9}{
%%		\draw [fill=red](0.0,\y) circle (0.1cm);
%%		\draw [fill=red](0.75,\y) circle (0.1cm);
%%		\draw [fill=red](5.25,\y) circle (0.1cm);
%%	}
%%	\foreach \x in {0.0,0.75,...,5.9}{
%%		\draw [fill=red](\x,0.0) circle (0.1cm);
%%		\draw [fill=red](\x,0.75) circle (0.1cm);
%%		\draw [fill=red](\x,5.25) circle (0.1cm);
%%	}
%	
%	\foreach \x in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](\x,0.75) circle (0.1cm);
%		\draw [fill=gray](\x,5.25) circle (0.1cm);
%	}
%	\foreach \y in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](5.25,\y) circle (0.1cm);
%		\draw [fill=gray](0.75,\y) circle (0.1cm);
%	}
%%	\draw [fill=none,color=black,ultra thick](3.0,3.0) circle (0.3cm);
%	
%	\end{tikzpicture}
%	\caption{Test}
%	\label{fig: IBMfig}
%\end{figure}{}


%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=0.85]
%	\fill[cpu1] (0.0,0.0) rectangle (7.5,7.5);
%	% \fill[cpu1] (6.0,0.0) rectangle (7.5,6.0);
%	\fill[cpu2] (0.75,4.5) rectangle (5.25,5.25);
%	\fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
%	\fill[cpu2] (0.75,0.75) rectangle (1.5,4.5);
%	\fill[cpu2] (4.5,0.75) rectangle (5.25,4.5);
%	\fill[cpu2] (0.0,1.5) rectangle (0.75,4.5);
%	\fill[cpu2] (5.25,1.5) rectangle (6.0,4.5);
%	\fill[cpu2] (1.50,0.0) rectangle (4.5,3.0);
%	% \fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
%	
%	% \fill[cpu2] (0.0,0.0) rectangle (6.0,1.5);
%	% \fill[cpu2] (0.0,1.5) rectangle (1.5,4.5);
%	% \fill[cpu2] (4.5,1.5) rectangle (6.0,4.5);
%	\fill[cpu4] (4.5,1.5) rectangle (1.5,4.5);
%	\fill[cpu4] (0.75,2.25) rectangle (1.5,3.75);
%	\fill[cpu4] (4.5,2.25) rectangle (5.25,3.75);
%	\fill[cpu4] (2.25,4.5) rectangle (3.75,5.25);
%	\fill[cpu4] (2.25,0.75) rectangle (3.75,1.5);
%	\draw[step=1.5cm, thick] (0,0) grid (7.5,7.5);
%	\draw[-,black, thick] (0,0.75) -- (6,0.75);
%	\draw[-,black, thick] (0,5.25) -- (6,5.25);
%	\draw[-,black, thick] (0.75,0) -- (0.75,6.0);
%	\draw[-,black, thick] (5.25,0) -- (5.25,6.0);
%	\draw[-,black, thick] (2.25,0) -- (2.25,1.5);
%	\draw[-,black, thick] (3.75,0) -- (3.75,1.5);
%	\draw[-,black, thick] (2.25,4.5) -- (2.25,6.0);
%	\draw[-,black, thick] (3.75,4.5) -- (3.75,6.0);
%	
%	\draw[-,black, thick] (0,2.25) -- (1.5,2.25);
%	\draw[-,black, thick] (0,3.75) -- (1.5,3.75);
%	
%	\draw[-,black, thick] (4.5,2.25) -- (6,2.25);
%	\draw[-,black, thick] (4.5,3.75) -- (6,3.75);
%	
%	% \fill[gray,opacity = 0.4 ] (3,3 ) circle (2.5cm);
%	\draw[red,ultra thick] (3,3 ) circle (2.5cm);
%	
%	% \fill[red,opacity = 0.2] (6.0,0.0) rectangle (7.5,6.0);
%	\foreach \x in {0,1.5,...,7.5}{
%		\draw [fill=red](\x,0.0) circle (0.1cm);
%		\draw [fill=red](\x,7.5) circle (0.1cm);
%		\draw [fill=red](\x,6.0) circle (0.1cm);
%	}
%	\foreach \y in {0,1.5,...,7.5}{
%		\draw [fill=red](0.0,\y) circle (0.1cm);
%		\draw [fill=red](6.0,\y) circle (0.1cm);
%		\draw [fill=red](7.5,\y) circle (0.1cm);
%	}
%	
%	\foreach \x in {1.5,3.0,4.5}
%	\foreach \y in {1.5,3.0,4.5}
%	\draw [fill=gray](\x,\y) circle (0.1cm);
%	
%	\foreach \y in {0.0,0.75,...,5.9}{
%		\draw [fill=red](0.0,\y) circle (0.1cm);
%		% \draw [fill=red](6.0,\y) circle (0.1cm);
%		\draw [fill=red](0.75,\y) circle (0.1cm);
%		\draw [fill=red](5.25,\y) circle (0.1cm);
%	}
%	\foreach \x in {0.0,0.75,...,5.9}{
%		\draw [fill=red](\x,0.0) circle (0.1cm);
%		\draw [fill=red](\x,0.75) circle (0.1cm);
%		\draw [fill=red](\x,5.25) circle (0.1cm);
%	}
%	
%	\foreach \x in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](\x,0.75) circle (0.1cm);
%		\draw [fill=gray](\x,5.25) circle (0.1cm);
%	}
%	\foreach \y in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](5.25,\y) circle (0.1cm);
%		\draw [fill=gray](0.75,\y) circle (0.1cm);
%	}
%	\draw [fill=none,color=black,ultra thick](3.0,3.0) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](3.0,4.5) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](3.0,1.5) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](1.5,3.0) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](4.5,3.0) circle (0.3cm);
%	% % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
%	% \node[align=left] at (1.5,-0.75) {\Intercepted};
%	
%	% \fill[blue,opacity = 0.2] (3.0,-0.9) rectangle (3.3,-0.6);
%	% \node[align=left] at (4.5,-0.75) {\Out};
%	
%	% \fill[black,opacity = 0.2] (6.0,-0.9) rectangle (6.3,-0.6);
%	% \node[align=left] at (6.7,-0.75) {\In};
%	% % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
%	% % \node at (1.5,-0.75) {\Intercepted};
%	
%	\end{tikzpicture}
%	\caption{Test}
%	\label{fig: IBMfig}
%\end{figure}{}

==> arxiv-pack-2/sections/error-analysis.tex <==
\section{Error analysis} \label{sec:errors}
\subsection{Non-parametric equation}
Below, we provide some estimates on the errors incurred by \diffnet{} in approximating a sought solution. Suppose the exact solution of equation \ref{eq:poisson-kl-intro} is $ \uExact $ and the solution obtained at the end of the training process is given by $ \uNeural $. Let us also define $ \uNeuralExactOpt $ as the best possible function in $ \spaceVtheta  $. Note that, this function may or may not be able to match $ \uDiscrete $, but it represents the theoretical best possible function in the neural network function class. On the other hand, $ \uNeuralExactOpt $ might be different than $ \uNeural $ too, if the optimization algorithm is not able to reach the optimum $ \tilde{\netparams} $. We try to bound the error $ \eGen = \uNeural - \uExact $ by first breaking down the total error into errors from different sources.

\begin{lemma} \label{thm:losses-converge}
	Let the loss value at the $ n^{th}$ iteration of algorithm \ref{alg:pde-instance} be $ J_n $. Then $ \lim\limits_{n\rightarrow\infty} J_n = J(\tilde{\netparams})$
\end{lemma}
\begin{proof}
	Need to prove it using convexity.
\end{proof}
\begin{lemma} \label{thm:opt-error-low-single-instance}
	Let problem \ref{eq:def:loss-functional-inner-product-form} be optimized by algorithm \ref{alg:pde-instance}. Then the optimization error  $ \norm{\eOpt} = \norm{\uNeural - \uNeuralExactOpt} < \epsilon$, for any $ \epsilon>0 $.
\end{lemma}
\begin{proof}
	\begin{align}
	\begin{split}
	J(\uNeural) &= \int_{\spatialD} \left[\half |\grad \uNeural |^2 - f\uNeural \right]d\xvec \\
	&= \int_{\spatialD} \left[\half |\grad \uNeuralExactOpt + \grad\eOpt |^2 - f(\uNeuralExactOpt + \eOpt) \right]d\xvec \ \ (\text{using}\ \eOpt=\uNeural-\uNeuralExactOpt) \\
	&= \int_{\spatialD} \left[\half |\grad \uNeuralExactOpt|^2 + \half |\grad \eOpt |^2 +\grad\uNeuralExactOpt\cdot\grad\eOpt - f(\uNeuralExactOpt + \eOpt) \right]d\xvec \\
	&= \int_{\spatialD}\left[ \half |\grad \uNeuralExactOpt |^2 - f\uNeuralExactOpt \right]d\xvec + \half\int_{\spatialD}|\grad\eOpt|^2 d\xvec + \int_{\spatialD}\left[ \grad\eOpt\cdot\grad\uNeuralExactOpt - f\eOpt \right]d\xvec \\
	&= J(\uNeuralExactOpt) + \half\norm{\eOpt}^2
	\end{split}
	\end{align}
	Thus, $ \norm{\eOpt}^2 \leq C\left[J(\uNeural) - J(\uNeuralExactOpt)\right] $ with $ C\geq 2 $. Using Lemma \ref{thm:losses-converge} now gives the required result.
\end{proof}

The following theorem provides an estimate on the network capacity.
\begin{theorem}\label{thm:network-approximation-capacity}
	Fix $p \in P$. Suppose $(\Lop_p,f)$ is any PDE system defined over a compact domain $D$ which is uniformly discretized with resolution $h$. Let $u^*_h$ be the true solution evaluated at the discretization points. Consider the hypothesis class:
	\begin{align}
		\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
	\end{align}
	defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(1/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.
\end{theorem}
\begin{proof}
	The proof follows a recent result by Bubeck et al.~\cite{bubeck2020-memorization}. Let the output resolution of the network be $n$. For a fixed $p$, consider the (linear) vector space spanned by all possible (perhaps uncountably many) basis functions of the form
	$$
	f(\cdot) = a^i_l \text{ReLU}(\langle w^i_l, \cdot \rangle + b_l)
	$$
	where $a,b,w$ are arbitrary real-valued weights. Since $i = 1, \ldots, n$, the span of this space is no more than $n$-dimensional and isomorphic to $\mathbb{R}^m$ for some $m \leq n$. Therefore, there is a set of no more than $n$ basis functions (i.e., $n$ neurons) that can be used to represent $u^*_{p}$ any fixed $p$. Assuming the dimension of $p$ is small, we have $n \lesssim 1/h$. Therefore, $k = \Omega(1/h)$ neurons are sufficient to reproduce $u^*_p$.
\end{proof}

Notice that the above theorem shows that there exist DiffNet architectures that exactly drive the modeling error down to zero. However, the proof is \emph{non-constructive}, and there is no obvious algorithm to find the basis functions that reproduce the solution at the evaluation points. 

Theorem \ref{thm:network-approximation-capacity} essentially allows us to choose the neural network parameter family $ \Theta $ such that $ \norm{\eCap} <\epsilon$ for any $ \epsilon>0 $. Since, we are free to choose the network architecture, we can always assume that
\begin{align}
	\norm{\eCap} = \norm{\uNeuralExactOpt - \uDiscrete} \leq \epsilon, \ \ \epsilon>0.
\end{align}
\begin{remark}
	\ab{Check if this remark is justified}
	\diffnet{} is designed to be agnostic to a neural network. Therefore, both fully connected neural network as well as convolutional neural networks can be used for the network approximation. Since a convolutional neural network can be interpreted as a special case of a fully connected network, the above estimate holds for all cases.
\end{remark}

For the third source of error, i.e., the error due to discretization using finite element method can be estimated from standard finite element analysis literature:
\begin{lemma}
	Assume that the basis functions $ \phi_i(\xvec) $ in \ref{eq:def:fem-function-approximation-0} are chosen such that $ \phi_i(\xvec)\in C^p(K) $ locally within each element $ K\in\mesh $. Then,
	\begin{align}
		\norm{\uDiscrete - \uExact} \leq C(D)h^{p+1}\norm{u}_{H^2}
	\end{align}
\end{lemma}
\begin{proof}
	We refer to standard texts such as \cite{brenner2007mathematical,hughes2012finite} for a proof.
\end{proof}

Finally we can write down the estimate for the generalization error in \diffnet{} in the form of the following theorem.
\begin{theorem} \label{thm:diffnet-errors-non-parametric}
	Consider any DiffNet architecture producing fields with grid spacing $h$. Let $\gH$ denote the hypothesis class of all networks obeying that architecture. Suppose that $\Theta \in \gH$ is a DiffNet trained using the finite element loss $J_{FEM}$ defined above. Then, its generalization error obeys:
	\begin{align} \label{eq:error-bound-non-parametric}
	\normVtheta{\eGen} \leq \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{align}
	where $\text{Err}_\Theta$ is a term that only depends on the DiffNet optimization procedure, and $\text{Err}_\gH$ only depends on the choice of hypothesis class $\gH$.
\end{theorem}
\begin{proof}
	The result is simply an application of the triangle inequality. Dropping the subscript $ \spaceVtheta $:
	\begin{align}
	\begin{split}
	\norm{\eGen} &= \norm{\uNeural - \uNeuralExactOpt + \uNeuralExactOpt - \uDiscrete + \uDiscrete - \uExact} \\
	&\leq \norm{\uNeural - \uNeuralExactOpt} + \norm{\uNeuralExactOpt - \uDiscrete} + \norm{\uDiscrete - \uExact} \\
	&= \norm{\eOpt} + \norm{\eCap} + \norm{\eDis} \\
	&= \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{split}
	\end{align}		
\end{proof}

\subsection{Parametric equation}
The above theorem is for a single parameter choice $p$. An identical argument can be extended to any DiffNet FDM loss constructed by sampling a \emph{finite} number (say $m$) of parameters from a distribution over $P$. We obtain the following corollary.

\textbf{Corollary}.\emph{Consider a finite-sample version of the FDM loss $J_{FDM}$ constructed by taking the average over $m$ parameter choices sampled from $P$. Consider the hypothesis class}:
$$\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
$$ 
\emph{defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(m/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.}

This corollary shows that a wide two-layer network exists that can reproduce any (finite) set of field solutions to a PDE system, as long as the width scales linearly in the cardinality of the set. Getting bounds independent of the cardinality is an interesting open question.

\begin{lemma} \label{thm:losses-converge-parametric}
	Let the loss value at the $ n^{th}$ iteration of algorithm \ref{alg:pde-parametric} be $ J_n $. Then $ \lim\limits_{n\rightarrow\infty} J_n = J(\tilde{\netparams})$
\end{lemma}
\begin{proof}
	Need to prove it using convexity.
\end{proof}
\begin{theorem} \label{thm:diffnet-errors-parametric}
	Consider any DiffNet architecture producing fields with grid spacing $h$. Let $\gH$ denote the hypothesis class of all networks obeying that architecture. Suppose that $\Theta \in \gH$ is a DiffNet trained using the finite element loss $J_{FEM}$ defined above. Then, its generalization error obeys:
	\begin{align} \label{eq:error-bound-parametric}
	\normVtheta{\eGen} \leq \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{align}
	where $\text{Err}_\Theta$ is a term that only depends on the DiffNet optimization procedure, and $\text{Err}_\gH$ only depends on the choice of hypothesis class $\gH$.
\end{theorem}
\begin{proof}
	The result is simply an application of the triangle inequality. Dropping the subscript $ \spaceVtheta $:
	\begin{align}
	\begin{split}
	\norm{\eGen} &= \norm{\uNeural - \uNeuralExactOpt + \uNeuralExactOpt - \uDiscrete + \uDiscrete - \uExact} \\
	&\leq \norm{\uNeural - \uNeuralExactOpt} + \norm{\uNeuralExactOpt - \uDiscrete} + \norm{\uDiscrete - \uExact} \\
	&= \norm{\eOpt} + \norm{\eCap} + \norm{\eDis} \\
	&= \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{split}
	\end{align}		
\end{proof}
%Let us denote the true solution by $ u_* (\mvec{x}, \omega) $ and the solution from the neural network training as $ u(\mvec{x}, \omega; \netparams) $. Clearly $u_* (\mvec{x}, \omega)\in V$. Then the error
%%\begin{align*}
%%\normVh{u_g-u_*} \leq \normVh{u_g-u_{h, opt}} + \normVh{u_{h, opt} - u_h} + \normVh{u_h-u_*}
%%\end{align*}
%\begin{align*}
%	\normVhtheta{\uNeural - \ustar} \leq \normVhtheta{\uNeural-\uNeuralExactOpt} + \normVhtheta{\uNeuralExactOpt - \uneuralDiscOmega} + \normVhtheta{\uneuralDiscOmega - \uneuralPerfOmega} + \normVhtheta{\uneuralPerfOmega - \ustar}
%\end{align*}
%where the functions on the right hand side are as follows (in the reverse order):
%\begin{itemize}
%	\item $ \uneuralDiscOmega $ is the function which is a discrete function in $ \spatialD $ as well as $ \Omega $, but still assuming a perfect network and perfect optimization.
%\end{itemize}
%
%%\ch{The first part needs to be estimated from the properties of the generator}
%%\begin{align*}
%%\normVh{u_g-u_h} < \epsilon
%%\end{align*}
%%\ch{The second part needs to be estimated from the properties of the optimization technique}:
%%\begin{align*}
%%\normVh{u_{h, opt} - u_h} < \epsilon
%%\end{align*}
%The third part can be estimated by the results from the a priori error analysis of Galerkin's method:
%\begin{align}
%\normVh{u_h-u_*} &= \int_{\Omega}\int_{D}(u_h - u_*)^2 d\mvec{a} d\mvec{x}\\
%&\leq \int_{A}C(\mvec{a})N_x^{-(p+1)}d\mvec{a}\\
%&\leq C_{max}N_x^{-(p+1)} \int_{A} d\mvec{a}\\
%&=C_{max}N_x^{-(p+1)}
%\end{align}
%where $ p $ is the degree of local basis function used for the FEM discretization and loss calculation.
%
%Finally we want to show that
%\begin{align*}
%\normVh{u_g-u_*} \leq C \xi(N_x, \alpha)
%\end{align*}


%\subsection{Generalization bounds: Special cases}
%We now examine a few special cases for which we can \emph{indeed} obtain concrete upper bounds on the DiffNet generalization error $E_D$. 
%
%It will be convenient to separately analyze the optimization and the modeling errors. Let us focus on the modeling error first. In this case, the nature of the bound will depend on the network architecture and/or type of the PDE system being analyzed. Because of a simple corollary of the universal approximation of neural networks, we get the following theorem:
%
%\textbf{Theorem}. \emph{Fix $p \in P$. Suppose $(\Lop_p,f)$ is any PDE system defined over a compact domain $D$ which is uniformly discretized with resolution $h$. Let $u^*_h$ be the true solution evaluated at the discretization points. Consider the hypothesis class}:
%$$\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
%$$ 
%\emph{defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(1/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.}
%
%\textbf{Proof sketch}. The proof follows a recent result by Bubeck et al.~\cite{bubeck2020-memorization}. Let the output resolution of the network be $n$. For a fixed $p$, consider the (linear) vector space spanned by all possible (perhaps uncountably many) basis functions of the form
%$$
%f(\cdot) = a^i_l \text{ReLU}(\langle w^i_l, \cdot \rangle + b_l)
%$$
%where $a,b,w$ are arbitrary real-valued weights. Since $i = 1, \ldots, n$, the span of this space is no more than $n$-dimensional and isomorphic to $\mathbb{R}^m$ for some $m \leq n$. Therefore, there is a set of no more than $n$ basis functions (i.e., $n$ neurons) that can be used to represent $u^*_{p}$ any fixed $p$. Assuming the dimension of $p$ is small, we have $n \lesssim 1/h$. Therefore, $k = \Omega(1/h)$ neurons are sufficient to reproduce $u^*_p$.
%\qed 
%
%
%Notice that the above theorem shows that there exist DiffNet architectures that exactly drive the modeling error down to zero. However, the proof is \emph{non-constructive}, and there is no obvious algorithm to find the basis functions that reproduce the solution at the evaluation points. 
%
%The above theorem is for a single parameter choice $p$. An identical argument can be extended to any DiffNet FDM loss constructed by sampling a \emph{finite} number (say $m$) of parameters from a distribution over $P$. We obtain the following corollary.
%
%\textbf{Corollary}.\emph{Consider a finite-sample version of the FDM loss $J_{FDM}$ constructed by taking the average over $m$ parameter choices sampled from $P$. Consider the hypothesis class}:
%$$\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
%$$ 
%\emph{defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(m/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.}
%
%This corollary shows that a wide two-layer network exists that can reproduce any (finite) set of field solutions to a PDE system, as long as the width scales linearly in the cardinality of the set. Getting bounds independent of the cardinality is an interesting open question.


==> arxiv-pack-2/sections/formulations-fdm-loss.tex <==
\subsubsection{Finite difference based loss function}\label{sec:loss-fdm}
Suppose the set $ \mvec{X} = (\mvec{x}_1,\mvec{x}_2,.., \mvec{x}_N) \in \mathbb{R}^{n\times N} $ denote a collection of points in $ \mathbb{R}^n $ that produces a (uniform) discretization of D. Define $ S_i = s(\mvec{x}_i) $ and $ U_i $ an approximation of the unknown $ u(\mvec{x}_i) $. And as usual, we also define the vectors $ \mvec{S} = (S_1,S_2,..,S_N) $ and $ \mvec{U} = (U_1,U_2,..,U_N) $. Note that, each $ U_i $ is a function of the network parameters, i.e., $ U_i = U_i(\mvec{\theta}) $ or $ \mvec{U} = \mvec{U}(\mvec{\theta}) $, where $ \mvec{\theta} $ denotes the network parameters.

On this regularly spaced stencil, the numerical derivatives can be approximately written in terms of finite difference formulas. 

\begin{align}\label{def:fdm-difference-equations}
	D^r u(\xii) \approx \sum_{j = -k_1}^{k_2} c_j(h) U_j
\end{align}
where $ D $ is a differential operator, $ r $ is the order or derivative, $ c $'s are known values (depends on the grid spacing $ h $) and $ U_i $ as explained above. $ k_1 $ and $ k_2 $ are some integers that follows the choice of the stencil.
Using the expressions of these finite difference formulas, we can then write the discrete PDE at each of the points in $ \mvec{X} $. By writing $ N $ such equations, we obtain an $ N $-dimensional linear system. For a linear PDE, this is easily written as:
\begin{subequations}\label{eq:fdm-equations-setup}
	\begin{align}
	a_{i1}U_1 + a_{i2}U_2  +\ldots +a_{iN}U_N = f_i, \quad i=1,2,...,N^{int}\label{eq:fdm-interior}
	\\
	b_{i1}U_1 + b_{i2}U_2  +\ldots +b_{iN}U_N = g_i, \quad i=1,2,...,N^{bc}\label{eq:fdm-boundary}
	\end{align}
\end{subequations}
Combining the interior and boundary equations, we can write down the matrix form,
\begin{align}\label{eq:fdm-linear-system-matrix-notation}
	\mmat{A}\text{ }\mvec{U} = \mvec{f}.
\end{align}
The residual vector $ \mvec{R}_{FDM} $ can be defined as
\begin{align}\label{def:fdm-residual-matrix-notation}
	\mvec{R}_{FDM} = \mmat{A}\text{ }\mvec{U} - \mvec{f}.
\end{align}
At this point, we recognize that $ \mvec{A} $ is a function of $ \mvec{S} $ whereas $ \mvec{U} $ is a function of both $ \mvec{S} $ and the network parameters $ \netparams $. Also, $ \mvec{R}_{FDM} $ refers to the residual corresponding to a single instance of $ \mvec{S} $. So, to train the network against all the available data of $ \mvec{S} $, we define the following loss function:
\begin{align}\label{def:fdm-loss-stochastic-expectation}
	L_{FDM} = \mathbb{E}_{\omega\sim \Omega} \left\| \mvec{R}_{FDM}[\mvec{S}(\omega),\mvec{U}(\mvec{S}(\omega);\netparams)] \right\|^2_2.
\end{align}
To calculate the expectation numerically over the sample space $ \Omega $, we use a finite quasi-random sample sequence (such as Sobol sequences)  and define the approximate/numerical loss function as $ \hat{L}_{FDM} $:
\begin{align}\label{def:fdm-loss-stochastic-numerical}
	\hat{L}_{FDM}(\netparams) = \frac{1}{N_s} \sum_{i = 1}^{N_s}\left\| \mvec{R}_{FDM}[\mvec{S}(\omega_i),\mvec{U}(\mvec{S}(\omega_i);\netparams)] \right\|^2_2.
\end{align}

The loss function defined in \ref{def:fdm-loss-stochastic-numerical} evaluates the loss when the problem data $ s $ is a function of the random variable $ \omega $ and therefore the dataset $ \{S_i\}_{i = 1,..,N_s} $ is generated by constructing the sequence $ \{\omega_i\}_{i=1,..,N_s} $. But this loss function can also be used in the case when the dataset is not governed by a known probability distribution. In that case, we simply use:
\begin{align}
	\hat{L}_{FDM}(\netparams) = \frac{1}{N_s} \sum_{i = 1}^{N_s}\left\| \mvec{R}_{FDM}[\mvec{S}_i,\mvec{U}(\mvec{S}_i;\netparams)] \right\|^2_2.
\end{align}

The loss function $ \hat{L}_{FDM} $ is now a function of $ \mvec{\theta} $, and we can minimize $ \hat{L}_{FDM} $ with respect to $ \mvec{\theta} $ to reach the optimum network parameters,
\begin{align}
	\netparams^* = \arg\min_{\netparams} \hat{L}_{FDM}(\netparams).
\end{align}
% add comment about nonlinear equations

==> arxiv-pack-2/sections/formulations-fem-loss.tex <==
\subsubsection{Finite element based loss function}\label{sec:loss-fem}
The finite element based loss function is inspired by the Galerkin formulation of an elliptic PDE as well as the Rayleigh-Ritz method. In this case, we actually construct a function of certain regularity in the domain variable $ \xvec $, as opposed to just assuming a function of certain differentiability at the collocation points, as was the case in Sec. \ref{sec:loss-fdm}.

Suppose $ H^1(D) = W^{1,2}(D) $ denotes the Sobolev space of functions whose first derivatives are square integrable. Define the space $ V $ as
\begin{align}\label{eq:def:function-space-V}
	V = \setbuilder{v\in H^1(D) : v(0,y) = 1, v(1,y) = 0}.
\end{align}
Then the Galerkin formulation of equation \ref{eq:poisson-kl-intro} is to find $ u\in V $ such that,
\begin{align}\label{eq:galerkin-formulation-poisson-kl}
	B(u,v) = L(v) \ \ \forall v\in V,
\end{align}
where,
\begin{subequations}\label{eq:def:bilnear-linear-form}
	\begin{align}
		B(u,v) &= \int_{\spatialD}(\grad v\cdot \grad u) d\xvec \\
		L(v) &= \int_{\spatialD} vf d\xvec.
	\end{align}
\end{subequations}

Equation \ref{eq:galerkin-formulation-poisson-kl} yields an algebraic equation for each function $ v $ taken from the space V. Thus, if $ V $ is discretized such that it can be represented by a finite basis, then the Galerkin formulation \ref{eq:galerkin-formulation-poisson-kl} yields a finite system of algebraic equations.

From the principle of variational formulation, it is also known that equation \ref{eq:galerkin-formulation-poisson-kl} is the Euler-Lagrange equation of the following functional $ J(u) $ of $ u \in V $:
\begin{align} \label{eq:def:loss-functional-inner-product-form}
	J(u) = \half B(u,u) - L(u).
\end{align}
Therefore, the solution $ u $ can also be written as the minimizer of the cost function $ J $:
\begin{align}\label{eq:minimization-problem-continuous}
	u = \argmin_{u\in V} J(u).
\end{align}

In \diffnet, we make use of this functional $ J $, but instead of minimizing it against the solution $ u $, we minimize it against the network parameters $ \theta $. Since $ V $ is an infinite dimensional space, we need to discretize it to a finite subspace where we can evaluate $ J $. For this, let $ \mesh $ be a discretization of $ \spatialD $ into $ \nel $ ``finite'' elements $ K_i $ such that $ \cup_{\nel}K_i = D $. Then the discrete function space $ V^h $ is define as:
\begin{align}
	V^h = \setbuilder{v^h \in V: v^h|_{K}\in P_m(K), \ K\in \mesh},
\end{align}
where $ P_m(K) $ denotes the set of polynomial functions of degree $ m $ define on $ K $. Let the dimension of $ V^h $ be $ N $, which essentially means that the number of unknowns in the domain is also $ N $. Suppose $ \{ \phi_i(\xvec) \}_{i = 1}^{N} $ is a suitable basis that span $ V^h $. Then any function $ \uh \in V^h $ can be written as
\begin{align}\label{eq:def:fem-function-approximation-0}
	\uh(\xvec) = \sum_{i = 1}^{N} \phi_i(\mvec{x})U_i,
\end{align}
where $ U_i $ are the function values at the nodal points in the mesh $ \mesh $. 
Then equation \ref{eq:minimization-problem-continuous} can be rewritten for $ \uh $ as:
\begin{align}\label{eq:minimization-problem-discrete}
	\uh = \argmin_{\uh \in V^h} J(\uh).
\end{align}

A minimization problem such as \ref{eq:minimization-problem-discrete} is known as the Rayleigh-Ritz method. But in the presence of a neural network, we minimize $ J $ with respect to the network parameter $ \netparams $ instead of $ \uh $. For this, we need to first explicitly state the $ \theta $ dependence of $ \uh $. This can be done by a slight modification to \ref{eq:def:fem-function-approximation-0} as below:
%Equation \ref{eq:def:fem-function-approximation-0} still needs to be made precise about the dependence on the the network parameter $ \theta $ as well as the network input $ s $. As in the case of the finite difference based method, each $ U_i $ is a function of the network parameter $ \netparams $. So the precise notation for \ref{eq:def:fem-function-approximation-0} is
\begin{align}\label{eq:def:fem-function-approximation-1}
	\uh(\xvec;\netparams) = \sum_{i = 1}^{N} \phi_i(\mvec{x})U_i(\theta),
\end{align}
along with a generalization of the function space $ V $ as:
\begin{align}\label{eq:def:function-space-V-theta}
	\spaceVtheta = \setbuilder{v(\theta)\in H^1(\spatialD):v(x=0,y;\netparams) = 1, v(x=1,y;\netparams)=0}.
\end{align}
Then we can finally write down the \diffnet{} solution $ \uh_{\netparams^*} $ in two steps:
\begin{subequations}\label{eq:minimization-problem-theta-1}
	\begin{align}
		\netparams^* &= \argmin_{\netparams \in \Theta} J(\uh(\xvec; \netparams)) \\
		\uh_{\netparams^*} &=  \uh(\xvec; \netparams^*)
	\end{align}
\end{subequations}

The discussion leading to \ref{eq:minimization-problem-theta-1} is based on a non-parametric diffusivity, i.e., $ \tilde{\diffusivity} = \diffusivity(\xvec) $. When the diffusivity is parameterized by $ \omega $, i.e., $ \tilde{\diffusivity} = \diffusivity(\xvec,\omega) $, then the function space $ V^h(\netparams) $ needs to be modified as:
\begin{align}\label{eq:def:function-space-V-theta-stochastic}
	V^h_\netparams = \setbuilder{v: \| v(\xvec,\omega; \netparams) \|_{V^h_{\netparams}} < \infty,\ v(x=0,y,\omega;\netparams) = 1, v(x=1,y,\omega;\netparams)=0}
\end{align}
where, $\|\cdot\|_{V^h_{\netparams}}$ is the energy norm
\begin{align}\label{eq:def:stochastic-norm}
	\|v\|_{V^h_{\netparams}}^2 = \mathbb{E}_{\omega\sim\Omega}\left[\int_D \nu(\mvec{x}, \omega; \netparams)|\nabla v|^2d\mvec{x}\right].
\end{align}
With this choice of function space, the FEM loss function can be written as:
\begin{align}\label{def:fem-loss-stochastic-expectation}
	L_{FEM}(\netparams) = \mathbb{E}_{\omega\in\Omega}J(\uh(\xvec, \omega; \netparams))
\end{align}

The right hand side of \ref{def:fem-loss-stochastic-expectation} involves two integrations: one over the spatial domain $ \spatialD $ and the other an expectation over $ \Omega $. The integration over $ \spatialD $ is evaluated numerically using Gaussian quadratures rules. And the expectation over $ \Omega $ is evaluated approximately by a summation over a finite number of samples, similar to \ref{def:fdm-loss-stochastic-numerical}, i.e.,
\begin{align}\label{def:fem-loss-stochastic-numerical}
	\hat{L}_{FEM}(\netparams) = \frac{1}{N_s}\sum_{i = 1}^{N_s}J(s(\omega), \uh(\xvec,\omega); \theta).
\end{align}

The loss function $ \hat{L}_{FEM}(\netparams) $ is now just a function of $ \netparams $ and we can minimize it with respect to $ \netparams $, just as in the case of $ \hat{L}_{FDM}(\netparams) $,
\begin{subequations}\label{eq:minimization-problem-theta-2}
	\begin{align}
		\label{eq:minimization-problem-theta-2-opt}
		\netparams^* &= \argmin_{\netparams \in \Theta} \hat{L}_{FEM}(\netparams) \\
		\label{eq:minimization-problem-theta-2-sol}
		\uh_{\netparams^*} &=  \uh(\xvec, \omega; \netparams^*).
	\end{align}
\end{subequations}
%The FEM involves the weakening of the PDE using an appropriate weighting functions. As in the FDM case, we consider a discretization of the domain $ D $ into a finite number of non-overlapping elements denoted by $ Q_i $, $ i = 1,2,\ldots,\nel $ such that $ \cup_{i}^{nel} Q_i = D $. The unknown solution can be approximated as:
%
%where $\phi_i$ are the finite element basis functions.

%FEM is essentially an integrated method. Since $ \uh(\mvec{x}) $ is not a collection of values any more (unlike FDM), an integration needs to be carried out in order to get rid of the explicit dependence on $ \mvec{x} $. This fact also gives a very natural hint on how to define the loss function.

%\bk{can we be more certain than might be here?}In fact, there might be multiple ways to define the loss function using FEM approximation. We discuss two of them below:

% \begin{itemize}
% 	\item \textbf{Non-weighted loss}\bk{better to remove this}
% 	\begin{align}
% 	\mathcal{N}(u;s) -f = 0
% 	\end{align}
% 	\begin{align}
% 	R_{\theta} = \left\| \mathcal{N}(u_{\theta};s) -f \right\|^2 = \int_{D} \left[ \mathcal{N}(u_{\theta};s) -f \right]^2 d\mvec{x}
% 	\end{align}
% 	Associated optimization problem:
% 	\begin{align}
% 	\theta^{*} &= \argmin_{\theta} \left\| \mathcal{N}(u_{\theta};s) -f \right\|^2 \\
% 	u^{*} &= u_{\theta^*}
% 	\end{align}
% 	This loss function uses the strong form of the PDE as opposed to the weak form, thus the differentiability of the basis functions must be higher than the highest order appearing in the PDE. In this current paper, we do not pursue this approach.
	
%This approximation is plugged into the PDE, after which we invoke Galerkin's method. That is, multiply the PDE with a test function and reduce the differentiability requirement on $ u^h $ via integration by parts \footnote{For completeness, we assume $u^h_{\theta} \in V \subset H^1(D)$ where $ H^1(D) $ denotes the Hilbert space of functions on $ D $ that have square integrable first derivatives,}:
%\begin{align}
%\int_{\Omega} v\left[ \mathcal{N}(u^h_{\theta};s) -f \right] d\mvec{x} &= 0 \text{ }\forall v\in V
%\end{align}
%Which results in this following (standard FEM) form
%\begin{align}
%B(v,u^h_{\theta}) - L(v) &= 0\text{ }\forall v\in V
%\end{align}
%where $B(v,u^h_{\theta})$ is the bilinear form that encodes the PDE, while $L(v)$ is the linear form that encodes the load and boundary conditions. By choosing the test function to be the (unknown) solution, $u^h_{\theta}$, we get an energy functional 
%\begin{align}
%J(u^h_{\theta}) = \frac{1}{2} B(u^h_{\theta},u^h_{\theta}) - L(u^h_{\theta}),
%\end{align}
%whose minima is the sought solution $ u^h_{\netparams^*} $, where
%\begin{align}
%	\netparams^* = \arg\min_{\netparams} J(u^h_\netparams).
%\end{align}
% 	Associated optimization problem:
% 	\begin{align}\label{def:fem-weighted-optimization}
% 	\theta^{*} &= \argmin_{\theta} J(u_{\theta}) \\
% 	u^{*} &= u_{\theta^*}\label{def:u-optimal}
% 	\end{align}
%\end{itemize}
% \bk{need to define $B, L$}
% $ J(u,u) $ has the interpretation of the energy of the system, and the optimization problem is similar to the minimum energy principle, the only difference being that the minimization in ~\ref{def:fem-weighted-optimization} is with respect to $ \theta $ instead of $ u $. \ch{} \bg{To Review}
%This energy functional accounts for the PDE as well as all Neumann (and Robin) conditions. This serves as our loss function.
%\subsection{Non-weighted loss}
%\begin{align}
%\mathscr{L}(u) -f = 0
%\end{align}
%\begin{align}
%R_{\theta} = \left\| \mathscr{L}(u_{\theta}) -f \right\|^2 = \int_{\Omega} \left[ \mathscr{L}(u_{\theta}) -f \right]^2 d\mvec{x}
%\end{align}
%Associated optimization problem:
%\begin{align}
%\theta^{*} &= \argmin_{\theta} \left\| \mathscr{L}(u_{\theta}) -f \right\|^2 \\
%u^{*} &= u_{\theta^*}
%\end{align}
%
%\subsection{Weighted loss}
%\begin{align}
%\mathscr{L}(u) -f = 0
%\end{align}
%Assuming $u_{\theta} \in V$
%\begin{align}
%\int_{\Omega} v\left[ \mathscr{L}(u_{\theta}) -f \right] d\mvec{x} &= 0 \text{ }\forall v\in V\\
%B(v,u) - L(v) &= 0\text{ }\forall v\in V
%\end{align}
%The corresponding energy functional is 
%\begin{align}
%J(u) = \frac{1}{2} B(u,u) - L(u)
%\end{align}
%Associated optimization problem:
%\begin{align}
%\theta^{*} &= \argmin_{\theta} J(u_{\theta}) \\
%u^{*} &= u_{\theta^*}
%\end{align}
% \textbf{Note} We have used the superscript $ d $ in a loose sense, to denote a discrete quantity in both FDM and FEM context. So in FDM context $ U^d_\theta $ just means a vector such as $ \mvec{U} = (U_1,U_2,..,U_N) $, whereas in the FEM context $ U^d_\theta $ can mean both the discrete function $ u^h $ (as in Equation \ref{def:fem-function-approximation}) or the unknown coefficients (nodal values) $ \mvec{U} = (U_1,U_2,..,U_N) $

==> arxiv-pack-2/sections/implementations.tex <==
\section{Implementations}

%\input{figure_panels/derivative-calc-illustration-fdm.tex}
\input{figure_panels/derivative-calc-illustration-fem.tex}

\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.99\linewidth]{images/UNetArch.png}
	\caption{UNet architecture used for training \invnet{}}
	\label{fig:unetarch}
\end{figure}

\subsection{Model architecture for \invnet{}}\label{sec:model-arch}
Due to the structured grid representation of $\mathcal{S}^d$ and similar structured representation of $U^d_\theta$, deep convolutional neural networks are a natural choice of network architecture. The spatial localization of convolutional neural networks helps in learning the interaction between the discrete points locally. Since, the network takes an input of a discrete grid representation (similar to an image, possibly with multiple channels) and predicts an output of the solution field of a discrete grid representation (similar to an image, possibly with multiple channels), this is considered to be similar to a image segmentation or image-to-image translation task in computer vision. U-Nets~\citep{ronneberger2015u,cciccek20163d} have been known to be effective for applications such as semantic segmentation and image reconstruction. Due to its success in diverse applications, we choose U-Net architecture for \invnet{}. The architecture of the network is shown in Figure~\ref{fig:unetarch}. First, a block of convolution, and instance normalization is applied. Then, the output is saved for later use during skip-connection. This intermediate output is then down sampled to a lower resolution for a subsequent block of convolution, instance normalization layers. This process is continued for two more times. Now, the upsampling starts where, the saved outputs of similar dimensions are concatenated with the output of upsampling for creating the skip-connections followed by a  convolution layer. LeakyReLU activation was used for all the intermediate layers. The final layer has a Sigmoid activation. 
% Next we explain the training procedure used for training \invnet{}.

\subsection{Applying boundary conditions}\label{sec:boundary-conditions}
In \invnet{}, the Dirichlet boundary conditions are applied exactly. The query result $ U^d_\theta $ from the network pertains only to the interior of the domain. The boundary conditions need to be taken into account separately. There are two ways of doing this:
\begin{itemize}
	\item Applying the boundary conditions exactly (this is possible only for Dirichlet conditions in FEM/FDM; and the zero-Neumann case in FEM)
	\item Taking the boundary conditions into account in the loss function, thereby applying them approximately.
\end{itemize}

We take the first approach of applying the Dirichlet conditions exactly (subject to the mesh). Since the network architecture is well suited for 2d and 3d matrices (which serve as adequate representation of discrete field in 2d/3d on regular geometry), the imposition of Dirichlet boundary conditions amounts to simply padding the matrix by the appropriate values. A zero-Neumann condition can be imposed by taking the ``edge values" of the interior and copying them as the padding.
A nonzero Neumann condition is slightly more involved in the FDM case since additional equations need to be constructed; but if using FEM loss, this can be done with another surface integration on the relevant boundary.

\subsection{Calculation of derivatives and integration}\label{sec:derivative-integal-calc-detail}
The derivatives in FDM are calculated by in-built convolution operations. \invnet{} takes an image representation of the input field and returns another image for the solution. Thus, the vector $ U^d_\theta $ is represented as a matrix (or image) in the code. There is an advantage of using this representation, which is that the derivative calculations can be made very fast using convolution operations. The stencil size determines the size of the kernel, and the FDM difference coefficients form the elements of the kernel. This convolution is only performed within the loss function, and thus has no relation to the convolutional neural network that is used to approximate the solution. See Figure ~\ref{fig:fdm-grid-example} and ~\ref{fig:fdm-5pt-laplacial-conv-example} for example.

The same goes for the integration process in FEM. The full domain integration (i.e., $ \int D $) is nothing but the simple sum of the integration over the individual elements (i.e., $ \sum_{i = 1}^{N_{el}} \int D_i $). This integration over an individual element is in turn the simple weighted sum of the integrand evaluated at the Gauss quadrature points. This evaluation at a single Gauss point can be represented as convolution. Thus, if there are 4 Gauss points in each element, then 4 convolution operations will evaluate the integrand at those points for each element. After that, we only need to sum across Gauss points first, then followed by a sum across elements. See Figure ~\ref{fig:fem-mesh-with-gauss-pt} and ~\ref{fig:fem-function-evaluation-at-single-gauss-pt} for example.


%$U^d_\theta$ is similarly the discrete (unknown) solution to the PDE. In case of FDM, $U^d_\theta$ would mean a collection of values $\underline{U}$; whereas, in case of FEM, ${U^d_\theta}$ will mean a linear combination of a finite number of polynomial functions. Here we use the superscript $ d $ to loosely denote a discrete quantity either in FDM or in FEM. But it should be kept in mind that in case of FDM, a quantity $ f^d $ is just a collection of real values $f^d_{FDM} = \underline{f} = (f_1,f_2,...,f_N)\in\mathbb{R}^{N} $, whereas when we say $ f^d $ in the FEM context, it really means a function in the form of $ f^d_{FEM} = f^h = \sum_{i = 1}^{N}N_i(\mvec{x})f_i : D\rightarrow \mathbb{R}$.



%\subsection{Linear Poisson equation in 2D}
%The Poisson equation is given by
%\begin{align}
%	\grad\cdot(\tilde{\nu}(\mvec{x})\grad u) &= 0 \text{  in  } D \\
%	u(0, y) &= 1 \\
%	u(1, y) &= 0 \\
%	\partialder{u}{n} &= 0 \text{ on other boundaries} 
%\end{align}
%
%The loss function:
%\begin{align}
%	R = \int \tilde{\nu}|\grad u|^2 d\mvec{x}
%\end{align}



%\subsection{Linear Heat equation in 1D+T}
%The linear heat equation is given by
%\begin{align}
%	\begin{cases}
%		u_t - \visco u_{xx} = f \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } \Gamma_s\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
%	\end{cases}
%\end{align}
%where $\visco = \visco (\underline{x},t)$ and the forcing $f = f(\underline{x},t)$.
%
%The loss function:
%\begin{align}
%	R_u = \int \left[uu_t + \visco \left( u_x \right)^2\right]dxdt
%\end{align}
%\begin{align}
%	R_{LS} &= \int \left(u_t - \visco u_{xx}\right)^2 dxdt \\
%	&= \int \left((u_t)^2 - 2\visco u_t u_{xx} + (\visco u_{xx})^2\right) dxdt \\
%	&= \int \left[(u_t)^2 + 2\visco u_x u_{xt}\right]dxdt
%\end{align}
%
%\begin{align}
%	R_{GLS} &= \int \left[uu_t + \visco \left( u_x \right)^2\right]dxdt + \int \tau u_t \left(u_t - \visco u_{xx}\right) dxdt \\
%	&= \int \left[uu_t + \visco \left( u_x \right)^2 + \tau (u_t)^2 + \tau \visco u_x u_{xt}\right]dxdt 
%\end{align}
%
%\subsection{Inviscid/Burgers equation in 1D+T}
%The Burgers' equation is given by
%\begin{align}
%	\begin{cases}
%		u_t + u u_x - \visco u_{xx} = f \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } \Gamma_s\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
%	\end{cases}
%\end{align}
%where $\visco = \visco (\underline{x},t)$ and the forcing $f = f(\underline{x},t)$.
%
%The FDM loss function:
%The FDM loss function:
%\begin{align}
%	R = \sum_{i}^{N_{xy}} \left\| \partialder{u^i}{t} + u^i\partialder{u^i}{x}\right\|^{2} + \sum_{i}^{N_{bn}}\gamma \left(\left\|u - u^b(\cdot, x_0)\right\|^2 + \left\|u - u^b(t_0,\cdot)\right\|^2\right)
%\end{align}
%
%\begin{equation}
%{\partial u \over \partial t} + u {\partial u \over \partial x} = 0
%\label{eq:Inviscid_Burgers}
%\end{equation}
%
%\begin{equation}
%u(x,t=0) = \frac{1}{2}(1 - cos(2\pi c x))
%\label{eq:initial-condition}
%\end{equation}
%where $c \ge 0$ is the parameter, and the domain of interest is the unit square, \newline
%$(x,t) \in \color{black}[0,1]\times[0,0.2]$.

%\subsection{First order wave equation}
%The wave equation is given by
%\begin{align}
%	\begin{cases}
%		\frac{\partial u}{\partial t} + a\frac{\partial u}{\partial x} = 0 \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } x=0\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0
%	\end{cases}
%\end{align}
%with $u_0(x) = e^{-\frac{(x-0.4)^2}{0.01}}$
%\begin{align}
%	R_{\theta} = \left\|\frac{\partial u}{\partial t} + a\frac{\partial u}{\partial x} \right\|^2
%\end{align}
%
%\subsection{Wave equation in 1D+T}
%The wave equation is given by
%\begin{align}
%	\begin{cases}
%		\frac{\partial^2 u}{\partial t^2} - c^2 \frac{\partial^2 u}{\partial x^2} = f \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } \Gamma_s\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
%		\partialder{u}{t} = v_0(\mvec{x}) & \text{on } \Gamma_0
%	\end{cases}
%\end{align}
%where $c$ is the wave velocity and the forcing $f = f(\underline{x},t)$.

==> arxiv-pack-2/sections/intro.tex <==
%\section{Reference Notes (will be deleted)}
%	
%	Solving PDEs with a neural network as an approximation, a priori fixed mesh - (\cite{lee1990neural,lagaris1998artificial,lagaris2000neural,malek2006numerical,rudd2015constrained})
%	
%	PINN - (\cite{raissi2018hidden,raissi2019physics,kharazmi2019variational})
%	
%	Data-Driven Identification of Parametric Partial Differential Equations - (\cite{rudy2019data})
%	
%	Data driven Eulerian - (\cite{tompson2017accelerating})
%	
%	Optimal weighting of PDE loss and BC loss - (\cite{van2020optimally})
%	
%	DGM, was published at the same time as PINN, but arguably received much lesser limelight (\cite{sirignano2018dgm})
%	
%	Full field solutions - (\cite{paganini2018calogan,botelho2020deep,zhu2019physics})
%	
%	Pointwise predictions - (\cite{yang2018physics,pang2019fpinns,karumuri2020simulator,han2018solving,michoski2019solving})
%	
%	General class of pdes - (\cite{zhu2019physics,sirignano2018dgm,yang2018physics})
%	
%	Improvement in numerical linear algebra and single instance of pde: (\cite{pang2019fpinns,karumuri2020simulator,hsieh2019learning,katrutsa2017deep,greenfeld2019learning})
%	
%	Variational energy based: (\cite{samaniego2020energy})
%	
%	%	In many science and engineering disciplines, solving partial differential equations has long 

\section{Introduction}
\begin{figure}[t!]
	\begin{tikzpicture}
	\draw (0, 0) node[inner sep=0] {\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{images/invnet-schematic.png}};
	\draw (-2.9, -1.8) node {$S^d$};
	\draw (2.9, -1.8) node {$U^d$};
	\draw (0.2, -1.8) node {$G_{nn}$};
	\draw (0.2, -2.5) node {(a)};
	\end{tikzpicture}\hfill
	% 	\label{fig:invnet-network-representation}
	% \end{figure}
	% 	\begin{figure}
	\begin{tikzpicture}
	\draw (0, 0) node[inner sep=0] {\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{images/pinn-schematic.png}};
	\draw (-3.0, -0.3) node {$\mvec{x}_i$};
	\draw (1.3, 0.4) node {$u_{i}$};
	\draw (4.0, -0.4) node {$\mathbb{R}$};
	\draw (1.8, -1.15) node {$a$};
	\draw (3.3, -1.1) node {$b$};
	\draw (0.2, -1.8) node {$G_{nn}$};
	\draw (0.2, -2.5) node {(b)};
	\end{tikzpicture}
	\caption{(a) In our \invnet{} approach, we train a neural network to produce a discretized field solution over a mesh. Such an approach offers a direct link to powerful PDE analysis techniques, at the cost of a larger network. (b) In contrast, neural methods (like \cite{lagaris1998artificial,raissi2019physics}) are trained to produce point predictions: $ \neuralMap : D\rightarrow \mathbb{R}$, which are easier to train, but more difficult to analyze.} 
	\label{fig:common-networks-for-pdesolve}
\end{figure}

Numerical methods -- finite difference methods (FDM), finite element methods (FEM), spectral methods -- for solving PDEs discretize the physical domain (into cells, elements, ect) and \textit{approximate} the solution over this discretized domain using select families of basis functions \cite{hughes2012finite,leveque2007finite,trefethen2000spectral}. There is well developed and elegant theory that connects the discretization of the domain (in terms of element/cell dimension, $h$) and the properties of the basis functions (in terms of polynomial order, $\alpha$) with the quality of the ensuing numerical solution to the PDE. In particular, numerical stability arguments and \textit{a priori} error estimates allow users to judiciously reason about accuracy, robustness, and convergence \cite{brenner2007mathematical,larson2013finite}. Such theoretical arguments rely on the spatial discretization of the domain, and properties of the basis functions. Here, we formulate loss functions and networks that produce field solutions of PDEs (\figref{fig:common-networks-for-pdesolve}(a))  -- to be analogous with numerical PDE solvers --  in contrast to current neural PDE solvers that predominantly produce point estimate (\figref{fig:common-networks-for-pdesolve}(b)). %The guiding principle opens up theoretical arguments f. 

%The common theme that runs through all these methods is the idea that, even if an exact infinite dimensional solution is practically unobtainable (except for some trivial problems), it is still possible to obtain a \textit{finite dimensional} solution that is ``close enough" to the exact one. But this goal of rendering the finite dimensional problem, also known as ``discretization", is achieved through different devices in all these methods, as can be guessed from their naming. FDM does this by discretizing the domain of the PDE into finite number of points; and then assuming the existence of certain derivatives on the exact solution, it then attempts to obtain the numerical values of the function corresponding to those discrete points of the domain. On the other hand, FEM takes a completely different route where not only the domain is discretized, but also the solution is represented as a linear combination of a finite number of piecewise basis functions. 	An important characteristic of such approaches is that the methods are designed by keeping in mind the topology of the domain. Locality of information is replicated through the discrete points. This is because, although the exact solution is a function of a continuous variable, the discrete solution is determined by its values at discrete points, which often interact locally. 
% But with the development of deep neural networks and the prolific success in adapting deep learning methods into many diverse problems, attempts have been made to apply deep learning methods to solve PDEs. Some of the early works in this direction attempted to solve ODEs using a neural network but mostly focused on the linear algebra aspect of the network, i.e., with an eye to leverage the optimization formulation available with such a neural network \cite{lee1990neural}. The idea of using using a feed forward network to obtain a mapping between the domain variable (say, $ \mvec{x} $) and the range variable (say, $ u $) followed very soon \cite{lagaris1998artificial,lagaris2000neural}. $ u $ was considered as comprising of two components, the ``interior" and the ``boundary" parts. Only ``interior" part was for the network to learn, whereas the ``boundary" part was chosen to satisfy the applied boundary conditions. Much deeper network has also been used, particularly to solve higher order ODEs and system of ODEs \cite{malek2006numerical,rudd2015constrained}.


In recent years data-driven \cite{rudy2019data,tompson2017accelerating} and data-free approaches \cite{raissi2019physics,kharazmi2019variational,sirignano2018dgm,yang2018physics,pang2019fpinns,karumuri2020simulator,han2018solving,michoski2019solving,samaniego2020energy} for solving PDEs have been proposed. Most of these models are designed for pointwise prediction, i.e., the networks in these cases simply take as input $ \mvec{x} $ and produces an output value of $ u $, thereby calculating the value of $ u $ at one particular point. Some of these methods satisfy/apply the boundary conditions exactly \cite{lee1990neural,lagaris1998artificial,malek2006numerical} and others do that in an approximate manner \cite{lagaris2000neural,raissi2019physics,sirignano2018dgm}. Many of these methods do not require a mesh, and thus rely on collocating points from the domain randomly. The methods that approximately satisfies the boundary conditions do so by adding a loss function with respect to the specified boundary conditions. It has been shown by \cite{van2020optimally,wang2020understanding} that these losses have to be carefully weighted, making this an non-trivial exercise in hyper parameter tuning. This underlines the difficulty of applying the boundary conditions in a neural network-based method (or simply neural method).

 %There has also been efforts at improving the numerical linear algebra aspect of a neural network tasked with the job of finding an approximate solution to a PDE.

 %So in essence, the modern neural methods take the view that a deep neural network can represent complicated functions, and thus attempt to approximate the solution of the PDE through the neural network. In a way this seems an improvement over the classical numerical methods, in that the discrete solution is approximated through a highly complicated and nonlinear mapping as opposed to a linear combination of local functions of limited differentiability (which may not be the case for the exact solution). But on the other hand, these neural methods do not take into account the domain topology, and thus the ``local'' nature of the solution and sparsity of matrices that comes naturally to the classical methods, is missing in the neural methods. In addition, imposition of boundary conditions can be difficult in neural methods.
 

\textbf{Contributions:} We build upon some recent efforts that train networks to predict the full-field solution \cite{paganini2018calogan,botelho2020deep,zhu2019physics}. The specific contributions of this paper are :
\begin{enumerate}
	\item We present an algorithm that is bridges traditional numerical methods with neural methods. The neural network is designed to map inputs to the discretized field solution $ u $. However, the neural network is \textit{not responsible} for ensuring the spatial differentiability of the solution. Rather, the discrete field solution relies on traditional numerical methods (and associated numerical differentiation and quadrature) for construction of the loss function. Such an approach allows natural incorporation of different boundary conditions, and allows \textit{a priori} error estimates.
    \item We define two loss functions based on FDM and FEM. By setting up the loss function this way, we create the function space with appropriate differentiability and also account for the ``local'' nature of the solution. 
    \item We demonstrate \invnet{}'s performance on linear Poisson equation in 2D and steady heat transfer.
\end{enumerate}
%  \item Using these two loss functions we develop a neural approximation framework, \invnet{}, for providing learning of the mapping for parametric PDEs.


==> arxiv-pack-2/sections/methods.tex <==
\section{Formulations}\label{sec:formulations}
\subsection{Neural approximation of the solution}\label{sec:neural-approximation-of-solution}
Instead of seeking a mapping between the domain and an interval on the real line (Fig.~\ref{fig:common-networks-for-pdesolve}(b)), we seek a mapping between the input $ s $ and the full field solution $ u $ in the discrete spaces (Fig.~\ref{fig:common-networks-for-pdesolve}(a)). $S^d$ denotes the discrete representation of the known quantity $s$. $S^d$ could be either available only at discrete points (perhaps from some experimental data); or in many cases, $s$ might be known in a functional form and thus $S^d$ will be simply the values of $s$  evaluated on the discrete points. Therefore, if we denote a \invnet{} (see Figure ~\ref{fig:common-networks-for-pdesolve}(a)) network by $ \neuralMap $, then $ \neuralMap $ takes as input a discrete or functional representation of $ s $ and outputs a discrete solution field $U^d_\theta$, where $\netparams$ denote the network parameters:
\begin{align}\label{def:neural-function-definition}
	U^d_\netparams = \neuralMap(S^d; \netparams)
\end{align}
%For example, if we consider a PDE defined on a 2D bounded domain, then $ \neuralMap $ simply takes a 2D matrix containing the values of $ s $ and returns the solution $ U^d_\theta $ which is also a 2D matrix.

An untrained network, as expected, will produce a mapping that does not satisfy the discrete PDE; in fact, it will show a huge error. Our goal is to bring this error down to an acceptable level, and thereby reaching a solution that is ``close enough" to the exact solution. And we do this by designing the loss function based on major ideas taken from the classical numerical methods. This is explained next.



\subsection{Loss functions inspired by numerical methods}\label{sec:loss-functions}
The design of the loss function, along with the choice of the neural mapping, forms the central part of our approach. As referenced before, the loss functions are based either on finite difference or on finite element discretization. We discuss both of these separately below.

%\input{sections/formulations-fdm-loss.tex}
\input{sections/formulations-fem-loss.tex}

\subsection{Training algorithm for \invnet{}}\label{sec:training-process}
We provide two versions of the training algorithm. (i) an algorithm for computing the solution for an instance of a PDE and (ii) an algorithm for approximating the solution for a parametric PDE. The model architecture and the loss function remain the same for both. For solution for an instance, we use a simple approach as explained in Algorithm~\ref{alg:pde-instance}. While sampling from a distribution of coefficients/forcing field for a parametric PDE, we employ the mini-batch based optimization approach as explained in Algorithm~\ref{alg:pde-parametric}. The sampling of the known quantities is performed by using Sobol sampling methodology. For training the neural network, we predict the solution field using sampled inputs and compute the loss using the FDM/FEM loss. We employ Adam optimizer with a learning rate of $1E-5$ for performing the optimization of the neural network parameters, $\theta$ using the gradients obtained from the FDM/FEM loss. 


%\begin{algorithm}[t]
%	\caption{Algorithm for an instance of a PDE}\label{alg:pde-instance}
%	\footnotesize
%	\begin{algorithmic}[1]
%		\STATE Initialize $ \neuralMap $, \textsc{tol}
%		
%		\FOR{\texttt{epoch} $ \leftarrow $ 1 to \texttt{max\_epoch}}
%		\STATE $U^d_\theta_{int} \gets G_{nn}(S^d)$ 
%		\COMMENT{``int" stands for interior nodes}
%		\STATE $U^d_\theta \gets U^d_\theta_{int}\chi_{int} + U^d_\theta_{bc}\chi_{b}$
%		\STATE $ L =  $
%		\ENDFOR 
%	\end{algorithmic}
%\end{algorithm}

\begin{algorithm}[t]
	\caption{Algorithm for an instance of a PDE}\label{alg:pde-instance}
	\begin{algorithmic}[1]
		\Require $ S^d $, $ (U^d_\theta)_{bc} $, $ \alpha $ and \textsc{tol}
		\State Initialize $ \neuralMap $		
		\For{\texttt{epoch} $ \leftarrow $ 1 to \texttt{max\_epoch}}
		\State $(U^d_\theta)_{int} \gets G_{nn}(S^d)$ 
		\Comment{``int" stands for interior nodes}
		\State $(U^d_\theta) \gets (U^d_\theta)_{int}\chi_{int} + (U^d_\theta)_{bc}\chi_{b}$
		\State  $loss = L(U^d_\theta)  $
		\State $ \theta \gets optimizer(\theta,\alpha,\grad_\theta(loss))$
		\EndFor		 		
	\end{algorithmic}
\end{algorithm}
\begin{algorithm}[t]
	\caption{Algorithm for parametric PDE}\label{alg:pde-parametric}
	\begin{algorithmic}[1]
		\Require $ S^d $, $ (U^d_\theta)_{bc} $, $ \alpha $ and \textsc{tol}
		\State Initialize $ \neuralMap $		
		\For{\texttt{epoch} $ \leftarrow $ 1 to \texttt{max\_epoch}}
		\For{\texttt{mb} $ \leftarrow $ 1 to \texttt{max\_mini\_batches}}
		\State Sample $S^d_{mb}$ from the set\\
		\State $(U^d_\theta)_{int,mb} \gets G_{nn}(S^d_{mb})$\\
		\Comment{``int" stands for interior nodes}
		\State $(U^d_\theta)_{mb} \gets (U^d_\theta)_{int,mb}\chi_{int} + (U^d_\theta)_{bc}\chi_{b}$
		\State  $loss_{mb} = L(U^d_\theta)  $
		\State $ \theta \gets optimizer(\theta,\alpha,\grad_\theta(loss_{mb})) $
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

==> arxiv-pack-2/sections/preliminaries.tex <==
\section{Mathematical Preliminaries}\label{sec:preliminaries}
Consider a bounded open (spatial) domain $D \in \mathbb{R}^n, n\geq 2$ with a Lipschitz continuous boundary $\Gamma = \partial D$. We will denote the domain variable as $\mvec{x}$, where the boldface denotes a vector or tuple of real numbers. In $ \mathbb{R}^n $, we have $ \mvec{x} = (x_1,x_2,\ldots,x_n) $; but for 2D and 3D domains, we will use the more common notation $ \mvec{x} = (x,y) $ and $ \mvec{x} = (x,y,z) $ respectively. Consider also a probability space $ (\Omega, F, P) $, where $ \Omega $ is the sample space, $ F $ is the $ \sigma $-algebra of the subsets of $ \Omega $ and $ P $, a probability measure.

On this domain $ D $, we consider an abstract PDE on the function $u: D\times \Omega \rightarrow \mathbb{R}$ as:

\begin{subequations}\label{pde:abstract-representation-continuous}
	\begin{align}
	\mathcal{N}[u; s(\mvec{x},\omega)] &=f(\mvec{x}),\quad \mvec{x}\in D,\ \omega\in\Omega \label{pde:abstract-equation}\\
	\mathcal{B}[u]&=g(\mvec{x}),\quad \mvec{x}\in\Gamma. \label{pde:abstract-bc}
	\end{align}
\end{subequations}
Here, $\mathcal{N}$ is a differential operator (possibly nonlinear) operating on a function $u$. The differential equation also depends on the data of the problem $s$ which in turn is a function of the domain variable $ \mvec{x} $ and parameter $ \omega $. Thus $ \mathcal{N} $ is essentially a family of PDE's parameterized by $ \omega $. $ \mathcal{B} $ is a boundary operator on $ u $. In general, there can be multiple boundary operators for different part of the boundary $ \Gamma $.

Given a PDE along with some boundary conditions, such as one presented in \ref{pde:abstract-representation-continuous}, the goal is to find a solution $ u $ that satisfies \ref{pde:abstract-representation-continuous} as accurately as possible. Previous works such as \cite{lagaris1998artificial,raissi2019physics,sirignano2018dgm} seek to find this exact mapping $u: D \rightarrow \mathbb{R}$. But as we present in the next section, we do not have to restrict ourselves to this mapping, and in fact, with the help of deep neural networks coupled with numerical methods, we can find other mappings to retrieve a discrete solution.

In this work, we will focus on the Poisson's equation with both Dirichlet and Neumann conditions applied on the boundaries, along with a heterogeneous and stochastic diffusivity:
\begin{align}\label{eq:poisson-pde}
	-\grad\cdot(\diffusivity(\mvec{x},\omega)\grad u) &= f(\mvec{x}) \text{  in  } D
\end{align}
along with the boundary conditions
\begin{align}
	u &= g \text{ on } {\Gamma_D}\label{eq:poisson-bc-dirichlet} \\
	\partialder{u}{n} &= h  \text{ on } {\Gamma_N} \label{eq:poisson-bc-neumann}
\end{align}
where $ \diffusivity $ is the \emph{permeability} (or \emph{diffusivity}) which depends on both $ \xvec $ and the random variable $ \omega $; and $ f $ is the forcing. In relation to Eq. \ref{pde:abstract-representation-continuous}, $ \diffusivity $ plays the role of the data $ s $. $ \Gamma_D $ and $ \Gamma_N $ are the boundaries of the domain $ D $ where Dirichlet and Neumann conditions are specified respectively. We will assume that $ \partial D = \Gamma = \Gamma_D \cup \Gamma_N$.

\subsection{Poisson's equation in heterogeneous media}\label{sec:poisson-kl-problem-intro}
We are mostly interested in the problem of a steady state mass (or heat) transfer through an inhomogeneous medium (material). This essentially means that the material has different properties at different points. The only material property appearing in the Poisson's equation (\ref{eq:poisson-pde}) is $ \nu(\mvec{x}) $, thus the inhomogeneity can be modeled by a spatially varying $ \nu $, i.e., $ \nu = \nu(\mvec{x}) $. The equation and the BC's are given by:
\begin{subequations}\label{eq:poisson-kl-intro}
	\begin{align}
		-\grad\cdot(\tilde{\nu}(\mvec{x})\grad u) &= 0 \text{  in  } D \\
		u(0, y) &= 1 \\
		u(1, y) &= 0 \\
		\partialder{u}{y}(x,0) &= 0 \\
		\partialder{u}{y}(x,1) &= 0
	\end{align}
\end{subequations}
where $ D $ is a hypercube domain in $ \mathbb{R}^n $, $ n = 2,3 $. The diffusivity/permeability $ \tilde{\diffusivity} $ is heterogeneous with respect to $ \xvec $ and is also parameterized by $ \omega\in\Omega $. The specific form of $ \tilde{\diffusivity} $ is given in \ref{def:poisson-nu-harmonic-expansion}. The stochastic description of $ \tilde{\diffusivity} $ is discussed below.



==> arxiv-pack-2/sections/results.tex <==
\section{Results}\label{sec:results}
%We present results from a canonical PDE in two and three dimensions. Specifically, we consider the Poisson equation.
%Numerical examples in this work are as follows:
%\begin{itemize}
%	\item Linear/Nonlinear Poisson (log permeability)	
%	\item Linear Heat equation in space-time
%	\item Inviscid/Viscid Burgers in space-time
%	\item Wave equation in space-time
%\end{itemize}

\subsection{Error convergence for a non-parametric Poisson problem} \label{sec:linear-poisson-manufactured}
At the outset, we want to validate the error bounds stated in section \ref{sec:errors}. To this end, we solve the following non-parametric Poisson's equation:
\begin{subequations}\label{eq:poisson-manufactured-pde}
	\begin{align}
	-\laplacian u &= f \ \ \text{in} \ \spatialD \subset \mathbb{R}^2 \\
	u &= 0 \ \ \text{on} \ \partial\spatialD,
	\end{align}
\end{subequations}
where $ D = [0,1]^2 $ is a two-dimensional square domain. The forcing is chosen as
\begin{align} \label{eq:poisson-mms-forcing}
	f = f(\mvec{x}) = f(x,y) = 2\pi^2\sin(\pi x) \sin(\pi y).
\end{align}
The exact solution to problem \ref{eq:poisson-manufactured-pde} with forcing \ref{eq:poisson-mms-forcing} is given by $ u_{ex}(x,y) = \sin(\pi x) \sin(\pi y) $. For solving this problem, we seek to train a \diffnet{} that can predict the solution $ u $ given the forcing $ f $. At the discrete level, the network takes input $ F^d $ and outputs $ U^d $. The loss function \ref{eq:def:loss-functional-inner-product-form} takes the concrete form:
% FDM based loss:
%\begin{align}\label{def:loss-fdm-poisson-manufactured}
%R = \sum_{i}^{N_{xy}} \| \grad\cdot[{\nu}(\mvec{x}^i]\grad u(\mvec{x}^i)) + f(\mvec{x}^i)\|^{2}
%\end{align}
\begin{align}\label{def:loss-fem-poisson-manufactured}
J(u) = \frac{1}{2} \int |\grad u|^2 d\mvec{x} - \int u f d\mvec{x}.
\end{align}
Fig. \ref{fig:poisson-manufactured-contours} shows the contours of the network input $ F^d $, output $ U^d $, the exact solution evaluated on the mesh $ \mesh $ (a $ 256\times 256 $ grid) and the error ($ U^d - U_{ex} $).
%\begin{figure*}[!htb]
%	\centering
%	%	\includegraphics[trim=100 0 619 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
%	\includegraphics[trim=150 5 100 10,clip,width=0.95\linewidth]{results_data/poisson-convergence/query_contour_0.png}
%	\caption{Solution to the linear Poisson's equation with forcing. From left to right: $f$, $u^h_\theta$, $u_{num}$ and ($u^h_\theta-u_{num}$). Here $u_{num}$ is a conventional numerical solution obtained through FEM. Diffusivity $\visco = 1$}
%	\label{fig:poisson-manufactured-contours-0}
%\end{figure*}
\begin{figure}[!htb]
	\centering
	\begin{minipage}{.7\textwidth}
		\centering
		\begin{tikzpicture}
		\begin{axis}[
		width=0.99\linewidth, % Scale the plot to \linewidth
		height=6cm,
		%grid=major, % Display a grid
		%grid style={line width=.1pt, draw=gray!50}, % Set the style
		xlabel={{\# step}}, % Set the labels
		ylabel={$\log_{10}(L)$},
		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
		x tick label style={rotate=0,anchor=north} % Display labels sideways
		]
%		\addplot+ [thick, mark=none] table[x expr={\thisrow{Step}},y expr={ln(\thisrow{Value})/ln(10)},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/run-version_5-tag-PDE_loss.csv};
		\addplot+ [thick, mark=none]
		table[x expr={\thisrow{Step}},y expr={ln(\thisrow{Value})/ln(10)},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/run-version_0-tag-PDE_loss.csv};
		\legend{$L_{FEM}$}
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{Loss \textit{vs} optimization steps for the losses \ref{def:loss-fdm-poisson-kl} and \ref{def:loss-fem-poisson-kl}}
\end{figure}
\begin{figure}[!htb]
	\centering
	%	\includegraphics[trim=100 0 619 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
	\includegraphics[trim=75 0 75 0,clip,width=0.95\linewidth]{results_data/poisson-convergence/mms-vis.png}
	\caption{Solution to the problem \ref{eq:poisson-manufactured-pde} with forcing \ref{eq:poisson-mms-forcing} on a $ 256\times 256  $ grid. (Left) the discrete forcing $ F^d $, (middle-left) the solution $ U^d $ obtained from a \diffnet{} with a U-net architecture, (middle-right) the exact solution $ u_{ex} = \sin(\pi x)\sin(\pi y) $ evaluated on the mesh, denoted $ U_{ex}^d $, (right) the error $ (U^d - U^d_{ex}) $.  From left to right: $f$, $u^h_\theta$, $u_{num}$ and ($u^h_\theta-u_{num}$). Note: $ \norm{u} = 0.499979 $, $ \norm{u_{ex}} = 0.5 $, $ \norm{u-u_{ex}} = 2.4\times 10^{-5} $.}
	\label{fig:poisson-manufactured-contours}
\end{figure}

To study convergence behavior, we repeat this procedure with varying mesh length $ h $, starting from $ h = \oneOver{8} $ and gradually decreasing $ h $ till $ h = \oneOver{256} $. The calculated errors for each resolution are reported in Fig. \ref{fig:convergence-plot-non-parametric}. 

Theorem \ref{thm:diffnet-errors-non-parametric} estimates the total error by the contributions from three individual sources of errors, namely, the error due to finite element discretization ($ \eDis $), the error due to network approximation capacity ($ \eCap $) and the error due to the optimization process ($ \eOpt $). Of these three error sources, $ \eDis $ maintains a particular relation to the discretization parameter $ h $ (i.e., the mesh size). The other two errors do not hold a straight-forward relation with the mesh size or the network parameters. Thus, we put the estimate \ref{eq:error-bound-non-parametric} to test by keeping both $ \eCap $ and $ \eOpt $ sufficiently low, so that the dominating error is the discretization error $ \eDis $.

\input{figure_panels/mms_conv.tex}

We illustrate this by running two sets of \diffnet{} simulations.
\begin{itemize}
	\item The first set is where we completely remove the neural network and optimize the loss directly with respect to the displacement variables $ \mvec{U}^h $, i.e.
	\begin{align}
		\uh = \argmin_{\uh \in \spaceVh} J(\uh),
	\end{align}
	which is nothing but a classic Rayleigh-Ritz optimization. The absence of a neural network eliminates the error $ \eCap $. So the total error is a combination of only $ \eDis $ and $ \eOpt $. The total errors from this algorithm are plotted against the mesh size  $ h $ in Fig. \ref{fig:convergence-plot-non-parametric} under the legend ``\diffnet{} (No network)''. We see that the error plot has a slope of 2.
		
	\item The second set uses a neural network. Thus the optimization statement is the same as presented in equation \ref{eq:minimization-problem-theta-2}. Therefore, as discussed in theorem \ref{thm:diffnet-errors-non-parametric}, the total error is a combination of all three errors indicated in. To illustrate the interplay between the individual components of errors in this case, the following two simple experiments were done:
	\begin{itemize}
		\item \textit{Keeping the network unchanged across all $ h $-levels}: If we choose a particular network and use it to solve equation \ref{eq:poisson-manufactured-pde}, then the errors do not necessarily decrease with a decrease in $ h $. As shown in Fig. \ref{fig:convergence-plot-non-parametric}, the errors actually increase when $ h>2^{-5} $. This reason for this behaviour is that, when $ h $ becomes low, the number of discrete unknowns in the mesh (i.e., $ U_i $'s in equation \ref{eq:def:fem-function-approximation-0}) increases. In fact, in this case, the number of basis functions / unknowns, $ N $  is exactly equal to $ \oneOver{h^2} $. As $ h $ decreases, the size of the output $ U_i $'s increase. But since the network remains the same, the discrete function space $ \spaceVh $ does not remain a subspace of $ \spaceVhtheta $ anymore. This network function class also needs to get bigger to accommodate all the possible functions at the lower values of $ h $. 
		\item \textit{Enhancing the network capacity with decreasing $ h $}: In the sister experiment, we increase the depth of the UNet, thereby increasing the capacity of the network, thus at every $ h $-level, the space $ \spaceVhtheta $ is large enough so that it is a superset of $ \spaceVh $. Our goal in this experiment is not to obtain the optimum superset of $ \spaceVh $, rather, we just look for one such superset $ \spaceVhtheta \supset \spaceVh $. The plot from this experiment shows a slope of 2, which means that both $ \eCap \approx 0 $ and $ \eOpt \approx 0 $, and the only dominant error is the discretization error $ \eDis $. The fact that $ \eOpt $ is negligible affirms that the optimization algorithm is able to find the correct optima within the function space.
	\end{itemize}
\end{itemize}
Fig. \ref{fig:convergence-plot-non-parametric} also shows a plot of errors obtained from solving the same problem using a conventional FEM code (using numerical linear algebra) for reference.

\subsection{Poisson's equation with parametric log permeability}\label{sec:results-poisson-kl-problem}
Our second illustration is the solution of the PDE defined in Sec \ref{sec:poisson-kl-problem-intro} (equation \ref{eq:poisson-kl-intro}), which is frequently used for simulating practical problems such as heat or mass transfer through an inhomogeneous media. We solve this problem in both 2D and 3D domains, i.e., $ D=[0,1]^2 $ as well as $ D=[0,1]^3 $; $ \tilde{\nu} $ is now a function of $ \mvec{x} = (x,y) $ and is also parametric, as mentioned in \ref{def:poisson-nu-harmonic-expansion}.

We seek a mapping of the form $ u = \neuralMap(\diffusivity) $, where $ \neuralMap $ denotes the neural network. So $ S^d $ refers to the discrete version of $ \diffusivity $. Following the principle of Karhunen-Loeve expansion as described in Sec. \ref{sec:poisson-kl-problem-intro}, the infinite dimensional random space is truncated into a finite dimensional space. Thereafter, a finite set of samples are prepared from this space for the training process. Suppose the number of samples is $ N_s $. Then the loss function takes the concrete form:
%\textbf{Note:} When the diffusivity is constant, the mapping between the forcing and the solution is linear (the previous example).  But the mapping between $ u $ and $\tilde{\nu} $ is not linear. This can also be seen since $ \tilde{\nu}  $ and $ u $ are multiplied together in the PDE.
%The loss function takes the concrete form:
%\begin{align}\label{def:loss-fdm-poisson-kl}
%R = \sum_{i}^{N_{xy}} \left\| \grad\cdot({\nu}(\mvec{x}^i)\grad u (\mvec{x}^i)) - f(\mvec{x}^i)\right\|^{2} 
%%+ \sum_{i}^{N_{bn}}\gamma \left\|\partialder{u}{n}\right\|^2
%\end{align}
\begin{align}\label{def:loss-fem-poisson-kl-concrete}
J = \oneOver{N_s} \sum_{i = 1}^{N_s} \int_{\spatialD} \tilde{\nu}_i(\xvec)|\grad u_i(\xvec)|^2 d\mvec{x},
\end{align}
where, $ u_i = \neuralMap(\diffusivity_i, \netparams) $.
Both Dirichlet and Neumann conditions are present in this equation. In \diffnet{}, the Dirichlet conditions are applied exactly. The zero-Neumann condition is also applied exactly at the continuous level, since the boundary integrals vanish at the continuous level (see equation \ref{eq:def:bilnear-linear-form}).

By optimizing the loss \ref{def:loss-fem-poisson-kl-concrete} as described in \ref{eq:minimization-problem-theta-2}, we attempt to  learn the distribution of the stochastic solution, given that the coefficients in the log permeability K-L sum come from a known range of values that depends on the parameter space $ \omega $. We truncate the K-L sum after 6 terms. These six coefficients form a six-dimensional space from which the coefficient tuples $ \{a_i\}_{i=1}^{6} $ can be drawn. The \diffnet{} is trained by selecting a finite number ($ N_s $) of pseudo-random samples from this 6-dimensional space. For the results shown below, we have taken $ N_s=65536 $. We used the Adam optimization algorithm, with a learning rate of $ 10^{-4} $. Once the network is trained, we can perform inference by evaluating the network mapping for any diffusivity $ \diffusivity $ taken from the sample space. To illustrate the nature of the input ($ \diffusivity $ or $ S^d $) and the solution ($ u $ or $ U^d $), we present an anecdotal (i.e., a non-special and random) set of $ S^d $ and $ U^d $ in Fig. \ref{fig:poisson-kl-contours-2}. A reference solution using a conventional FEM program is also presented therein. Furthermore, sectional line cuts for these contours are shown in Figure \ref{fig:line-cuts-kl-2d-single}. The line cuts display a close match between \diffnet{} and the numerical reference solution.
\begin{figure}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/g_inp_contour.png}}
	\end{minipage}
	%	\begin{minipage}{.24\textwidth}
	%		\centering
	%		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
	%		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/fdm/u_gen_contour.png}}
	%	\end{minipage}	
	\begin{minipage}{.32\textwidth}
		\centering
		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/fem/u_gen_contour.png}}
	\end{minipage}
	\begin{minipage}{.32\textwidth}
		\centering
		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/num/u_num.png}}
	\end{minipage}	
	\caption{(Left) contours of $ \nu $ corresponding to $ \underline{\omega} = (-1,2,1.5,-1.3) $, (middle) \diffnet{} with an FEM based loss, (right) reference numerical solution using FEM}
	\label{fig:poisson-kl-contours-2}
\end{figure}
\input{figure_panels/kl_line_cuts_2d.tex}
%\begin{figure}
%	\centering
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		width=0.99\linewidth, % Scale the plot to \linewidth
%		%height=6cm,
%		%grid=major, % Display a grid
%		%grid style={line width=.1pt, draw=gray!50}, % Set the style
%		xlabel={$ y $}, % Set the labels
%		ylabel={$ u $},
%		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%		x tick label style={rotate=0,anchor=north} % Display labels sideways
%		]
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/u_lcut_x_13.txt};
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/u_lcut_x_13.txt};
%		\legend{\tiny{$L_{FDM}$}, \tiny{$L_{FEM}$}}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		width=0.99\linewidth, % Scale the plot to \linewidth
%		%height=6cm,
%		%grid=major, % Display a grid
%		%grid style={line width=.1pt, draw=gray!50}, % Set the style
%		xlabel={$ x $}, % Set the labels
%		ylabel={$ u $},
%		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%		x tick label style={rotate=0,anchor=north} % Display labels sideways
%		]
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/u_lcut_x_33.txt};
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/u_lcut_x_33.txt};
%		\legend{\tiny{$L_{FDM}$}, \tiny{$L_{FEM}$}}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		width=0.99\linewidth, % Scale the plot to \linewidth
%		%height=6cm,
%		%grid=major, % Display a grid
%		%grid style={line width=.1pt, draw=gray!50}, % Set the style
%		xlabel={$ x $}, % Set the labels
%		ylabel={$ u $},
%		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%		x tick label style={rotate=0,anchor=north} % Display labels sideways
%		]
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/u_lcut_x_52.txt};
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/u_lcut_x_52.txt};
%		\legend{\tiny{$L_{FDM}$}, \tiny{$L_{FEM}$}}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\caption{Dumb pictures of loss values}
%\end{figure}


%\begin{figure}[!htb]
%	\centering
%	%	\includegraphics[trim=100 0 619 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
%	\includegraphics[trim=0 0 0 0,clip,width=0.70\linewidth]{results_data/poisson-convergence/loss_all_annotated.png}
%	\caption{Loss plots for different resolutions}
%\end{figure}
% \subsubsection{Convergence studies}\label{sec:convergence-studies}
% To \ab{}


% \begin{figure}[!htb]
% \centering
% \begin{minipage}{.49\textwidth}
%   \centering
%  \begin{tikzpicture}
%      \begin{axis}[
%          width=0.99\linewidth, % Scale the plot to \linewidth
%          %grid=major, % Display a grid
%          %grid style={line width=.1pt, draw=gray!50}, % Set the style
%          xlabel= {\# step}, % Set the labels
%          ylabel=$\log_{10}(L)$,
%          legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%          x tick label style={rotate=0,anchor=north} % Display labels sideways
%       ]
%       \addplot [thick, mark=none]
%       table[x expr={\thisrow{Step}},y expr={ln(\thisrow{Value})/ln(10)},col sep=comma]{results_data/steady-heat-kl/loss_values.csv};
%      \end{axis}
%   \end{tikzpicture}
% \end{minipage}
%  \caption{Convergence of the error in $L^2$ norm for the Poissson equation with analytical solution $u =\sin{(\pi x)}\sin{(\pi y}$)}
% \end{figure}

%\subsubsection{In 2-D}
%4 terms in the K-L sum. 

% \begin{figure}[!htb]
% 	\centering
% 	%	\includegraphics[trim=652 0 100 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
% 	\includegraphics[trim={652 0 120 0},clip,width=0.98\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_15.png}
% 	\caption{Solution plot on horizontal line cuts at $y = 0.2, 0.5, 0.8$}
% 	\label{fig:poisson-kl-line-cuts-y}
% \end{figure}
\input{figure_panels/stochastic_histogram_panel.tex}
\subsubsection{Statistical distribution of solution}\label{sec:statistical-dist}
Since equation \ref{eq:poisson-kl-intro} is parametric, we can compare the quality of solution from \diffnet{} with a reference numerical solution in a statistical manner. We choose some points on the domain $ \spatialD $ (shown by markings on Fig. \ref{fig:query-points-for-statistics}) and evaluate the solution values at those query points for $ 20,000 $ samples of $ \diffusivity $. Therefore , at a particular query point, those $ 20,000 $ solution values approximately represent a distribution of the solution values at that point. So, we create a histogram of the solution values at each query point.
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[trim=0 0 0 0,clip,width=0.35\linewidth]{results_data/run_003-fem-sobol-query/histogram_query_points.png}
%	\caption{Query points for histogram analysis}
%	\label{fig:query-points-for-statistics-0}
%\end{figure}


The histograms are shown in Figure~\ref{fig:stochastic-histograms}. We notice a very close match between the histograms obtained from \diffnet{} and a conventional FEM solver. This once again confirms that \diffnet{} is effective in providing the correct statistics of the parametric Poisson equation.


%\input{tables/sample-size-study.tex}

\subsubsection{3-D Poisson's equation}
So far, we have focused on two-dimensional problems. Although 2D problems are useful in demonstrating the key features and properties of \diffnet{} method, most of the real problems are three-dimensional. \ab{Please check the next statement} \diffnet{} can solve both 2D and 3D problems without much changes to the architecture. In Fig. \ref{fig:poisson-kl-3d-contours}, we show one randomly selected pair of $ \diffusivity $ and $ u $ for a 3D problem obtained using \diffnet{}.
\begin{figure*}[!htb]
	\centering
	\includegraphics[trim=90 0 800 400,clip,width=0.3\linewidth]{results_data/steady-heat-kl/nu_3d.png}
	\includegraphics[trim=90 0 700 400,clip,width=0.4\linewidth]{results_data/steady-heat-kl/nu_3d_sliced_view.png}
	\\
	\includegraphics[trim=90 0 800 400,clip,width=0.3\linewidth]{results_data/steady-heat-kl/u_3d.png}
	\includegraphics[trim=90 0 700 400,clip,width=0.4\linewidth]{results_data/steady-heat-kl/u_3d_sliced_view.png}
	\caption{Example of $\nu(x,y,z)$ and the solution $u^h_{\theta}(x,y,z)$ to the 3D Poisson's problem with log permeability}
	\label{fig:poisson-kl-3d-contours}
\end{figure*}



%\input{figure_panels/old_pyplot_histograms.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{(Possible exclusion) Steady reaction-diffusion equation}\label{sec:steady-reaction-diffusion}
% \begin{align}\label{eq:reaction-diffusion-steady}
% -\grad\cdot({\nu}(\mvec{x})\grad u) + \kappa^2 u &= f \text{  in  } D \\
% u|_{\partial \Omega} &= 0
% \end{align}
%
% The loss function:
% \begin{align}\label{def:loss-fem-reaction-diffusion}
% R = \int \left[{\nu}|\grad u|^2 + \kappa^2 u^2 - fu \right] d\mvec{x}
% \end{align}
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/reaction-diffusion/kappa-50/query_contour_0.png}
% 	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/reaction-diffusion/kappa-100/query_contour_0.png}
% 	\caption{An example of solution of equation ~\ref{eq:reac-diff} for $\kappa = 50$ (top row) and $\kappa = 100$ (bottom row). From left to right: $f$, $u_{gen}$, $u_{num}$, $(u_{gen}-u_{num})$}
% \end{figure}
%
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[trim=140 0 645 0,clip,width=0.5\linewidth]{results_data/reaction-diffusion/kappa-50/query_line_cut_0.png}
% 	\caption{Solution plot on vertical line cuts at $x = 0.2, 0.5, 0.8$}
% \end{figure}
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[trim=651 0 120 0,clip,width=0.5\linewidth]{results_data/reaction-diffusion/kappa-50/query_line_cut_0.png}
% 	\caption{Solution plot on horizontal line cuts at $y = 0.2, 0.5, 0.8$}
% \end{figure}

==> arxiv-pack-2/sections/temp-error-analysis.tex <==
Nothing

==> figure_panels/old_pyplot_histograms.tex <==
\begin{figure}[!htb]
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1000.png} 
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1011.png}\\
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1021.png}
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1031.png}\\
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line1042.png}
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2122.png}\\
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2133.png}
		\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2143.png}
\end{figure}

\begin{figure}[!htb]
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line871.png} 
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line890.png}\\
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line910.png}
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2125.png}\\
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2144.png}
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line2164.png}\\
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line3445.png}
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line3464.png}
	\caption{XXXXXX}
\end{figure}
\begin{figure}[!htb]
	\includegraphics[trim=0 0 0 0,clip,width=0.48\linewidth]{results_data/pdf-fem-all/hist_u_line3484.png}
	\caption{YYYYYYYYY}
\end{figure}

==> sections/conclusions.tex <==
\section{Conclusions}
In this paper, we integrate neural PDE methods with numerical methods by performing numerical differentiation (and integration, if needed) instead of using the spatial differentiability. We defined two loss functions (based on FDM and FEM), for obtaining the neural approximate mapping between inputs and the discretized field solution. We demonstrate this framework's performance on poisson equation in 2D, steady heat transfer. We see that the results obtained from the neural PDE approximation (predicted) are match very closely with actual ground truth numerical solution. 


Remark: Pro-Con discussion of this approach versus conventional PINN
\begin{itemize}
    \item Con: From point prediction to field prediction $ => $ larger model
    \item Pro: Leverage rich theory of numerical analysis ..
\end{itemize}

%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=0.85]
%	\newcommand\reclenH{3}
%	\newcommand\reclenV{4}
%	\newcommand\ndiv{4}
%	\newcommand\stepsize{1}
%	\newcommand\xl{0}
%	\newcommand\yl{0}
%	\newcommand\osx{-0.5}
%	\newcommand\osy{0.5}
%	\fill[cpu2] (\xl,\yl) rectangle (\xl+\reclenH,\yl+\reclenV);
%	\draw[step=\stepsize cm] (\xl,\yl) grid (\xl+\reclenH,\yl+\reclenV);
%%	\draw (0, 0) node {$test$};
%	
%	\foreach \y in {0,1,2,3,4}{
%		\draw [fill=red](0,\y) circle (0.1cm);
%		\draw [fill=red](1,\y) circle (0.1cm);
%		\draw [fill=red](2,\y) circle (0.1cm);
%		\draw [fill=red](3,\y) circle (0.1cm);
%	}
%
%	\draw (\osx, 0) node {$e$};
%	\draw (\osx, 1) node {$d$};
%	\draw (\osx, 2) node {$c$};
%	\draw (\osx, 3) node {$b$};
%	\draw (\osx, 4) node {$a$};
%	
%	\draw (0,\reclenV + \osy) node {$1$};
%	\draw (1,\reclenV + \osy) node {$2$};
%	\draw (2,\reclenV + \osy) node {$3$};
%	\draw (3,\reclenV + \osy) node {$4$};
%	\end{tikzpicture}
%	\caption{Test}
%	\label{fig: IBMfig}
%\end{figure}{}

%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=0.85]
%	\fill[cpu1] (0.0,0.0) rectangle (8,8);
%	\fill[cpu1] (0.0,0.0) rectangle (7.5,7.5);
%	 \fill[cpu1] (6.0,0.0) rectangle (7.5,6.0);
%	\fill[cpu2] (0.75,4.5) rectangle (5.25,5.25);
%	\fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
%	\fill[cpu2] (0.75,0.75) rectangle (1.5,4.5);
%	\fill[cpu2] (4.5,0.75) rectangle (5.25,4.5);
%	\fill[cpu2] (0.0,1.5) rectangle (0.75,4.5);
%	\fill[cpu2] (5.25,1.5) rectangle (6.0,4.5);
%	\fill[cpu2] (1.50,0.0) rectangle (4.5,3.0);
%	
%	\fill[cpu4] (4.5,1.5) rectangle (1.5,4.5);
%	\fill[cpu4] (0.75,2.25) rectangle (1.5,3.75);
%	\fill[cpu4] (4.5,2.25) rectangle (5.25,3.75);
%	\fill[cpu4] (2.25,4.5) rectangle (3.75,5.25);
%	\fill[cpu4] (2.25,0.75) rectangle (3.75,1.5);
%	
%	\draw[step=1.5cm, thick] (0,0) grid (7.5,7.5);
%	\draw[-,black, thick] (0,0.75) -- (6,0.75);
%	\draw[-,black, thick] (0,5.25) -- (6,5.25);
%	\draw[-,black, thick] (0.75,0) -- (0.75,6.0);
%	\draw[-,black, thick] (5.25,0) -- (5.25,6.0);
%	\draw[-,black, thick] (2.25,0) -- (2.25,1.5);
%	\draw[-,black, thick] (3.75,0) -- (3.75,1.5);
%	\draw[-,black, thick] (2.25,4.5) -- (2.25,6.0);
%	\draw[-,black, thick] (3.75,4.5) -- (3.75,6.0);
%	
%	\draw[-,black, thick] (0,2.25) -- (1.5,2.25);
%	\draw[-,black, thick] (0,3.75) -- (1.5,3.75);
%	
%	\draw[-,black, thick] (4.5,2.25) -- (6,2.25);
%	\draw[-,black, thick] (4.5,3.75) -- (6,3.75);
%	
%	\draw[red,ultra thick] (3,3 ) circle (2.5cm);
%	
%%	\foreach \x in {0,1.5,...,7.5}{
%%		\draw [fill=red](\x,0.0) circle (0.1cm);
%%		\draw [fill=red](\x,7.5) circle (0.1cm);
%%		\draw [fill=red](\x,6.0) circle (0.1cm);
%%	}
%%	\foreach \y in {0,1.5,...,7.5}{
%%		\draw [fill=red](0.0,\y) circle (0.1cm);
%%		\draw [fill=red](6.0,\y) circle (0.1cm);
%%		\draw [fill=red](7.5,\y) circle (0.1cm);
%%	}
%	
%	\foreach \x in {1.5,3.0,4.5}
%	\foreach \y in {1.5,3.0,4.5}
%	\draw [fill=gray](\x,\y) circle (0.1cm);
%	
%%	\foreach \y in {0.0,0.75,...,5.9}{
%%		\draw [fill=red](0.0,\y) circle (0.1cm);
%%		\draw [fill=red](0.75,\y) circle (0.1cm);
%%		\draw [fill=red](5.25,\y) circle (0.1cm);
%%	}
%%	\foreach \x in {0.0,0.75,...,5.9}{
%%		\draw [fill=red](\x,0.0) circle (0.1cm);
%%		\draw [fill=red](\x,0.75) circle (0.1cm);
%%		\draw [fill=red](\x,5.25) circle (0.1cm);
%%	}
%	
%	\foreach \x in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](\x,0.75) circle (0.1cm);
%		\draw [fill=gray](\x,5.25) circle (0.1cm);
%	}
%	\foreach \y in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](5.25,\y) circle (0.1cm);
%		\draw [fill=gray](0.75,\y) circle (0.1cm);
%	}
%%	\draw [fill=none,color=black,ultra thick](3.0,3.0) circle (0.3cm);
%	
%	\end{tikzpicture}
%	\caption{Test}
%	\label{fig: IBMfig}
%\end{figure}{}


%\begin{figure}
%	\centering
%	\begin{tikzpicture}[scale=0.85]
%	\fill[cpu1] (0.0,0.0) rectangle (7.5,7.5);
%	% \fill[cpu1] (6.0,0.0) rectangle (7.5,6.0);
%	\fill[cpu2] (0.75,4.5) rectangle (5.25,5.25);
%	\fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
%	\fill[cpu2] (0.75,0.75) rectangle (1.5,4.5);
%	\fill[cpu2] (4.5,0.75) rectangle (5.25,4.5);
%	\fill[cpu2] (0.0,1.5) rectangle (0.75,4.5);
%	\fill[cpu2] (5.25,1.5) rectangle (6.0,4.5);
%	\fill[cpu2] (1.50,0.0) rectangle (4.5,3.0);
%	% \fill[cpu2] (1.50,5.25) rectangle (4.5,6.0);
%	
%	% \fill[cpu2] (0.0,0.0) rectangle (6.0,1.5);
%	% \fill[cpu2] (0.0,1.5) rectangle (1.5,4.5);
%	% \fill[cpu2] (4.5,1.5) rectangle (6.0,4.5);
%	\fill[cpu4] (4.5,1.5) rectangle (1.5,4.5);
%	\fill[cpu4] (0.75,2.25) rectangle (1.5,3.75);
%	\fill[cpu4] (4.5,2.25) rectangle (5.25,3.75);
%	\fill[cpu4] (2.25,4.5) rectangle (3.75,5.25);
%	\fill[cpu4] (2.25,0.75) rectangle (3.75,1.5);
%	\draw[step=1.5cm, thick] (0,0) grid (7.5,7.5);
%	\draw[-,black, thick] (0,0.75) -- (6,0.75);
%	\draw[-,black, thick] (0,5.25) -- (6,5.25);
%	\draw[-,black, thick] (0.75,0) -- (0.75,6.0);
%	\draw[-,black, thick] (5.25,0) -- (5.25,6.0);
%	\draw[-,black, thick] (2.25,0) -- (2.25,1.5);
%	\draw[-,black, thick] (3.75,0) -- (3.75,1.5);
%	\draw[-,black, thick] (2.25,4.5) -- (2.25,6.0);
%	\draw[-,black, thick] (3.75,4.5) -- (3.75,6.0);
%	
%	\draw[-,black, thick] (0,2.25) -- (1.5,2.25);
%	\draw[-,black, thick] (0,3.75) -- (1.5,3.75);
%	
%	\draw[-,black, thick] (4.5,2.25) -- (6,2.25);
%	\draw[-,black, thick] (4.5,3.75) -- (6,3.75);
%	
%	% \fill[gray,opacity = 0.4 ] (3,3 ) circle (2.5cm);
%	\draw[red,ultra thick] (3,3 ) circle (2.5cm);
%	
%	% \fill[red,opacity = 0.2] (6.0,0.0) rectangle (7.5,6.0);
%	\foreach \x in {0,1.5,...,7.5}{
%		\draw [fill=red](\x,0.0) circle (0.1cm);
%		\draw [fill=red](\x,7.5) circle (0.1cm);
%		\draw [fill=red](\x,6.0) circle (0.1cm);
%	}
%	\foreach \y in {0,1.5,...,7.5}{
%		\draw [fill=red](0.0,\y) circle (0.1cm);
%		\draw [fill=red](6.0,\y) circle (0.1cm);
%		\draw [fill=red](7.5,\y) circle (0.1cm);
%	}
%	
%	\foreach \x in {1.5,3.0,4.5}
%	\foreach \y in {1.5,3.0,4.5}
%	\draw [fill=gray](\x,\y) circle (0.1cm);
%	
%	\foreach \y in {0.0,0.75,...,5.9}{
%		\draw [fill=red](0.0,\y) circle (0.1cm);
%		% \draw [fill=red](6.0,\y) circle (0.1cm);
%		\draw [fill=red](0.75,\y) circle (0.1cm);
%		\draw [fill=red](5.25,\y) circle (0.1cm);
%	}
%	\foreach \x in {0.0,0.75,...,5.9}{
%		\draw [fill=red](\x,0.0) circle (0.1cm);
%		\draw [fill=red](\x,0.75) circle (0.1cm);
%		\draw [fill=red](\x,5.25) circle (0.1cm);
%	}
%	
%	\foreach \x in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](\x,0.75) circle (0.1cm);
%		\draw [fill=gray](\x,5.25) circle (0.1cm);
%	}
%	\foreach \y in {2.25,3.0,...,4.2}{
%		\draw [fill=gray](5.25,\y) circle (0.1cm);
%		\draw [fill=gray](0.75,\y) circle (0.1cm);
%	}
%	\draw [fill=none,color=black,ultra thick](3.0,3.0) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](3.0,4.5) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](3.0,1.5) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](1.5,3.0) circle (0.3cm);
%	%  \draw [fill=none,color=black,thick](4.5,3.0) circle (0.3cm);
%	% % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
%	% \node[align=left] at (1.5,-0.75) {\Intercepted};
%	
%	% \fill[blue,opacity = 0.2] (3.0,-0.9) rectangle (3.3,-0.6);
%	% \node[align=left] at (4.5,-0.75) {\Out};
%	
%	% \fill[black,opacity = 0.2] (6.0,-0.9) rectangle (6.3,-0.6);
%	% \node[align=left] at (6.7,-0.75) {\In};
%	% % \fill[red,opacity = 0.2] (0.0,-0.9) rectangle (0.3,-0.6);
%	% % \node at (1.5,-0.75) {\Intercepted};
%	
%	\end{tikzpicture}
%	\caption{Test}
%	\label{fig: IBMfig}
%\end{figure}{}

==> sections/error-analysis.tex <==
\section{Error analysis} \label{sec:errors}
\subsection{Non-parametric equation}
Below, we provide some estimates on the errors incurred by \diffnet{} in approximating a sought solution. Suppose the exact solution of equation \ref{eq:poisson-kl-intro} is $ \uExact $ and the solution obtained at the end of the training process is given by $ \uNeural $. Let us also define $ \uNeuralExactOpt $ as the best possible function in $ \spaceVtheta  $. Note that, this function may or may not be able to match $ \uDiscrete $, but it represents the theoretical best possible function in the neural network function class. On the other hand, $ \uNeuralExactOpt $ might be different than $ \uNeural $ too, if the optimization algorithm is not able to reach the optimum $ \tilde{\netparams} $. We try to bound the error $ \eGen = \uNeural - \uExact $ by first breaking down the total error into errors from different sources.

\begin{lemma} \label{thm:losses-converge}
	Let the loss value at the $ n^{th}$ iteration of algorithm \ref{alg:pde-instance} be $ J_n $. Then $ \lim\limits_{n\rightarrow\infty} J_n = J(\tilde{\netparams})$
\end{lemma}
\begin{proof}
	Need to prove it using convexity.
\end{proof}
\begin{lemma} \label{thm:opt-error-low-single-instance}
	Let problem \ref{eq:def:loss-functional-inner-product-form} be optimized by algorithm \ref{alg:pde-instance}. Then the optimization error  $ \norm{\eOpt} = \norm{\uNeural - \uNeuralExactOpt} < \epsilon$, for any $ \epsilon>0 $.
\end{lemma}
\begin{proof}
	\begin{align}
	\begin{split}
	J(\uNeural) &= \int_{\spatialD} \left[\half |\grad \uNeural |^2 - f\uNeural \right]d\xvec \\
	&= \int_{\spatialD} \left[\half |\grad \uNeuralExactOpt + \grad\eOpt |^2 - f(\uNeuralExactOpt + \eOpt) \right]d\xvec \ \ (\text{using}\ \eOpt=\uNeural-\uNeuralExactOpt) \\
	&= \int_{\spatialD} \left[\half |\grad \uNeuralExactOpt|^2 + \half |\grad \eOpt |^2 +\grad\uNeuralExactOpt\cdot\grad\eOpt - f(\uNeuralExactOpt + \eOpt) \right]d\xvec \\
	&= \int_{\spatialD}\left[ \half |\grad \uNeuralExactOpt |^2 - f\uNeuralExactOpt \right]d\xvec + \half\int_{\spatialD}|\grad\eOpt|^2 d\xvec + \int_{\spatialD}\left[ \grad\eOpt\cdot\grad\uNeuralExactOpt - f\eOpt \right]d\xvec \\
	&= J(\uNeuralExactOpt) + \half\norm{\eOpt}^2
	\end{split}
	\end{align}
	Thus, $ \norm{\eOpt}^2 \leq C\left[J(\uNeural) - J(\uNeuralExactOpt)\right] $ with $ C\geq 2 $. Using Lemma \ref{thm:losses-converge} now gives the required result.
\end{proof}

The following theorem provides an estimate on the network capacity.
\begin{theorem}\label{thm:network-approximation-capacity}
	Fix $p \in P$. Suppose $(\Lop_p,f)$ is any PDE system defined over a compact domain $D$ which is uniformly discretized with resolution $h$. Let $u^*_h$ be the true solution evaluated at the discretization points. Consider the hypothesis class:
	\begin{align}
		\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
	\end{align}
	defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(1/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.
\end{theorem}
\begin{proof}
	The proof follows a recent result by Bubeck et al.~\cite{bubeck2020-memorization}. Let the output resolution of the network be $n$. For a fixed $p$, consider the (linear) vector space spanned by all possible (perhaps uncountably many) basis functions of the form
	$$
	f(\cdot) = a^i_l \text{ReLU}(\langle w^i_l, \cdot \rangle + b_l)
	$$
	where $a,b,w$ are arbitrary real-valued weights. Since $i = 1, \ldots, n$, the span of this space is no more than $n$-dimensional and isomorphic to $\mathbb{R}^m$ for some $m \leq n$. Therefore, there is a set of no more than $n$ basis functions (i.e., $n$ neurons) that can be used to represent $u^*_{p}$ any fixed $p$. Assuming the dimension of $p$ is small, we have $n \lesssim 1/h$. Therefore, $k = \Omega(1/h)$ neurons are sufficient to reproduce $u^*_p$.
\end{proof}

Notice that the above theorem shows that there exist DiffNet architectures that exactly drive the modeling error down to zero. However, the proof is \emph{non-constructive}, and there is no obvious algorithm to find the basis functions that reproduce the solution at the evaluation points. 

Theorem \ref{thm:network-approximation-capacity} essentially allows us to choose the neural network parameter family $ \Theta $ such that $ \norm{\eCap} <\epsilon$ for any $ \epsilon>0 $. Since, we are free to choose the network architecture, we can always assume that
\begin{align}
	\norm{\eCap} = \norm{\uNeuralExactOpt - \uDiscrete} \leq \epsilon, \ \ \epsilon>0.
\end{align}
\begin{remark}
	\ab{Check if this remark is justified}
	\diffnet{} is designed to be agnostic to a neural network. Therefore, both fully connected neural network as well as convolutional neural networks can be used for the network approximation. Since a convolutional neural network can be interpreted as a special case of a fully connected network, the above estimate holds for all cases.
\end{remark}

For the third source of error, i.e., the error due to discretization using finite element method can be estimated from standard finite element analysis literature:
\begin{lemma}
	Assume that the basis functions $ \phi_i(\xvec) $ in \ref{eq:def:fem-function-approximation-0} are chosen such that $ \phi_i(\xvec)\in C^p(K) $ locally within each element $ K\in\mesh $. Then,
	\begin{align}
		\norm{\uDiscrete - \uExact} \leq C(D)h^{p+1}\norm{u}_{H^2}
	\end{align}
\end{lemma}
\begin{proof}
	We refer to standard texts such as \cite{brenner2007mathematical,hughes2012finite} for a proof.
\end{proof}

Finally we can write down the estimate for the generalization error in \diffnet{} in the form of the following theorem.
\begin{theorem} \label{thm:diffnet-errors-non-parametric}
	Consider any DiffNet architecture producing fields with grid spacing $h$. Let $\gH$ denote the hypothesis class of all networks obeying that architecture. Suppose that $\Theta \in \gH$ is a DiffNet trained using the finite element loss $J_{FEM}$ defined above. Then, its generalization error obeys:
	\begin{align} \label{eq:error-bound-non-parametric}
	\normVtheta{\eGen} \leq \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{align}
	where $\text{Err}_\Theta$ is a term that only depends on the DiffNet optimization procedure, and $\text{Err}_\gH$ only depends on the choice of hypothesis class $\gH$.
\end{theorem}
\begin{proof}
	The result is simply an application of the triangle inequality. Dropping the subscript $ \spaceVtheta $:
	\begin{align}
	\begin{split}
	\norm{\eGen} &= \norm{\uNeural - \uNeuralExactOpt + \uNeuralExactOpt - \uDiscrete + \uDiscrete - \uExact} \\
	&\leq \norm{\uNeural - \uNeuralExactOpt} + \norm{\uNeuralExactOpt - \uDiscrete} + \norm{\uDiscrete - \uExact} \\
	&= \norm{\eOpt} + \norm{\eCap} + \norm{\eDis} \\
	&= \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{split}
	\end{align}		
\end{proof}

\subsection{Parametric equation}
The above theorem is for a single parameter choice $p$. An identical argument can be extended to any DiffNet FDM loss constructed by sampling a \emph{finite} number (say $m$) of parameters from a distribution over $P$. We obtain the following corollary.

\textbf{Corollary}.\emph{Consider a finite-sample version of the FDM loss $J_{FDM}$ constructed by taking the average over $m$ parameter choices sampled from $P$. Consider the hypothesis class}:
$$\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
$$ 
\emph{defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(m/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.}

This corollary shows that a wide two-layer network exists that can reproduce any (finite) set of field solutions to a PDE system, as long as the width scales linearly in the cardinality of the set. Getting bounds independent of the cardinality is an interesting open question.

\begin{lemma} \label{thm:losses-converge-parametric}
	Let the loss value at the $ n^{th}$ iteration of algorithm \ref{alg:pde-parametric} be $ J_n $. Then $ \lim\limits_{n\rightarrow\infty} J_n = J(\tilde{\netparams})$
\end{lemma}
\begin{proof}
	Need to prove it using convexity.
\end{proof}
\begin{theorem} \label{thm:diffnet-errors-parametric}
	Consider any DiffNet architecture producing fields with grid spacing $h$. Let $\gH$ denote the hypothesis class of all networks obeying that architecture. Suppose that $\Theta \in \gH$ is a DiffNet trained using the finite element loss $J_{FEM}$ defined above. Then, its generalization error obeys:
	\begin{align} \label{eq:error-bound-parametric}
	\normVtheta{\eGen} \leq \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{align}
	where $\text{Err}_\Theta$ is a term that only depends on the DiffNet optimization procedure, and $\text{Err}_\gH$ only depends on the choice of hypothesis class $\gH$.
\end{theorem}
\begin{proof}
	The result is simply an application of the triangle inequality. Dropping the subscript $ \spaceVtheta $:
	\begin{align}
	\begin{split}
	\norm{\eGen} &= \norm{\uNeural - \uNeuralExactOpt + \uNeuralExactOpt - \uDiscrete + \uDiscrete - \uExact} \\
	&\leq \norm{\uNeural - \uNeuralExactOpt} + \norm{\uNeuralExactOpt - \uDiscrete} + \norm{\uDiscrete - \uExact} \\
	&= \norm{\eOpt} + \norm{\eCap} + \norm{\eDis} \\
	&= \text{Err}_\Theta + \text{Err}_\gH + O(h^\alpha)
	\end{split}
	\end{align}		
\end{proof}
%Let us denote the true solution by $ u_* (\mvec{x}, \omega) $ and the solution from the neural network training as $ u(\mvec{x}, \omega; \netparams) $. Clearly $u_* (\mvec{x}, \omega)\in V$. Then the error
%%\begin{align*}
%%\normVh{u_g-u_*} \leq \normVh{u_g-u_{h, opt}} + \normVh{u_{h, opt} - u_h} + \normVh{u_h-u_*}
%%\end{align*}
%\begin{align*}
%	\normVhtheta{\uNeural - \ustar} \leq \normVhtheta{\uNeural-\uNeuralExactOpt} + \normVhtheta{\uNeuralExactOpt - \uneuralDiscOmega} + \normVhtheta{\uneuralDiscOmega - \uneuralPerfOmega} + \normVhtheta{\uneuralPerfOmega - \ustar}
%\end{align*}
%where the functions on the right hand side are as follows (in the reverse order):
%\begin{itemize}
%	\item $ \uneuralDiscOmega $ is the function which is a discrete function in $ \spatialD $ as well as $ \Omega $, but still assuming a perfect network and perfect optimization.
%\end{itemize}
%
%%\ch{The first part needs to be estimated from the properties of the generator}
%%\begin{align*}
%%\normVh{u_g-u_h} < \epsilon
%%\end{align*}
%%\ch{The second part needs to be estimated from the properties of the optimization technique}:
%%\begin{align*}
%%\normVh{u_{h, opt} - u_h} < \epsilon
%%\end{align*}
%The third part can be estimated by the results from the a priori error analysis of Galerkin's method:
%\begin{align}
%\normVh{u_h-u_*} &= \int_{\Omega}\int_{D}(u_h - u_*)^2 d\mvec{a} d\mvec{x}\\
%&\leq \int_{A}C(\mvec{a})N_x^{-(p+1)}d\mvec{a}\\
%&\leq C_{max}N_x^{-(p+1)} \int_{A} d\mvec{a}\\
%&=C_{max}N_x^{-(p+1)}
%\end{align}
%where $ p $ is the degree of local basis function used for the FEM discretization and loss calculation.
%
%Finally we want to show that
%\begin{align*}
%\normVh{u_g-u_*} \leq C \xi(N_x, \alpha)
%\end{align*}


%\subsection{Generalization bounds: Special cases}
%We now examine a few special cases for which we can \emph{indeed} obtain concrete upper bounds on the DiffNet generalization error $E_D$. 
%
%It will be convenient to separately analyze the optimization and the modeling errors. Let us focus on the modeling error first. In this case, the nature of the bound will depend on the network architecture and/or type of the PDE system being analyzed. Because of a simple corollary of the universal approximation of neural networks, we get the following theorem:
%
%\textbf{Theorem}. \emph{Fix $p \in P$. Suppose $(\Lop_p,f)$ is any PDE system defined over a compact domain $D$ which is uniformly discretized with resolution $h$. Let $u^*_h$ be the true solution evaluated at the discretization points. Consider the hypothesis class}:
%$$\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
%$$ 
%\emph{defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(1/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.}
%
%\textbf{Proof sketch}. The proof follows a recent result by Bubeck et al.~\cite{bubeck2020-memorization}. Let the output resolution of the network be $n$. For a fixed $p$, consider the (linear) vector space spanned by all possible (perhaps uncountably many) basis functions of the form
%$$
%f(\cdot) = a^i_l \text{ReLU}(\langle w^i_l, \cdot \rangle + b_l)
%$$
%where $a,b,w$ are arbitrary real-valued weights. Since $i = 1, \ldots, n$, the span of this space is no more than $n$-dimensional and isomorphic to $\mathbb{R}^m$ for some $m \leq n$. Therefore, there is a set of no more than $n$ basis functions (i.e., $n$ neurons) that can be used to represent $u^*_{p}$ any fixed $p$. Assuming the dimension of $p$ is small, we have $n \lesssim 1/h$. Therefore, $k = \Omega(1/h)$ neurons are sufficient to reproduce $u^*_p$.
%\qed 
%
%
%Notice that the above theorem shows that there exist DiffNet architectures that exactly drive the modeling error down to zero. However, the proof is \emph{non-constructive}, and there is no obvious algorithm to find the basis functions that reproduce the solution at the evaluation points. 
%
%The above theorem is for a single parameter choice $p$. An identical argument can be extended to any DiffNet FDM loss constructed by sampling a \emph{finite} number (say $m$) of parameters from a distribution over $P$. We obtain the following corollary.
%
%\textbf{Corollary}.\emph{Consider a finite-sample version of the FDM loss $J_{FDM}$ constructed by taking the average over $m$ parameter choices sampled from $P$. Consider the hypothesis class}:
%$$\gH := \{ u_\Theta : p \mapsto \sum_{l=1}^k a^{i}_l \text{ReLU}(\langle w^{i}_l, p \rangle + b^{i}_l), i=1,\ldots,n. \}
%$$ 
%\emph{defined as the set of all two-layer neural networks with $k$ hidden neurons equipped with ReLU activation. Then, as long as $k = \Omega(m/h)$, there exists a network in $\gH$ for which $\text{Err}_\gH = 0$.}
%
%This corollary shows that a wide two-layer network exists that can reproduce any (finite) set of field solutions to a PDE system, as long as the width scales linearly in the cardinality of the set. Getting bounds independent of the cardinality is an interesting open question.


==> sections/formulations-fdm-loss.tex <==
\subsubsection{Finite difference based loss function}\label{sec:loss-fdm}
Suppose the set $ \mvec{X} = (\mvec{x}_1,\mvec{x}_2,.., \mvec{x}_N) \in \mathbb{R}^{n\times N} $ denote a collection of points in $ \mathbb{R}^n $ that produces a (uniform) discretization of D. Define $ S_i = s(\mvec{x}_i) $ and $ U_i $ an approximation of the unknown $ u(\mvec{x}_i) $. And as usual, we also define the vectors $ \mvec{S} = (S_1,S_2,..,S_N) $ and $ \mvec{U} = (U_1,U_2,..,U_N) $. Note that, each $ U_i $ is a function of the network parameters, i.e., $ U_i = U_i(\mvec{\theta}) $ or $ \mvec{U} = \mvec{U}(\mvec{\theta}) $, where $ \mvec{\theta} $ denotes the network parameters.

On this regularly spaced stencil, the numerical derivatives can be approximately written in terms of finite difference formulas. 

\begin{align}\label{def:fdm-difference-equations}
	D^r u(\xii) \approx \sum_{j = -k_1}^{k_2} c_j(h) U_j
\end{align}
where $ D $ is a differential operator, $ r $ is the order or derivative, $ c $'s are known values (depends on the grid spacing $ h $) and $ U_i $ as explained above. $ k_1 $ and $ k_2 $ are some integers that follows the choice of the stencil.
Using the expressions of these finite difference formulas, we can then write the discrete PDE at each of the points in $ \mvec{X} $. By writing $ N $ such equations, we obtain an $ N $-dimensional linear system. For a linear PDE, this is easily written as:
\begin{subequations}\label{eq:fdm-equations-setup}
	\begin{align}
	a_{i1}U_1 + a_{i2}U_2  +\ldots +a_{iN}U_N = f_i, \quad i=1,2,...,N^{int}\label{eq:fdm-interior}
	\\
	b_{i1}U_1 + b_{i2}U_2  +\ldots +b_{iN}U_N = g_i, \quad i=1,2,...,N^{bc}\label{eq:fdm-boundary}
	\end{align}
\end{subequations}
Combining the interior and boundary equations, we can write down the matrix form,
\begin{align}\label{eq:fdm-linear-system-matrix-notation}
	\mmat{A}\text{ }\mvec{U} = \mvec{f}.
\end{align}
The residual vector $ \mvec{R}_{FDM} $ can be defined as
\begin{align}\label{def:fdm-residual-matrix-notation}
	\mvec{R}_{FDM} = \mmat{A}\text{ }\mvec{U} - \mvec{f}.
\end{align}
At this point, we recognize that $ \mvec{A} $ is a function of $ \mvec{S} $ whereas $ \mvec{U} $ is a function of both $ \mvec{S} $ and the network parameters $ \netparams $. Also, $ \mvec{R}_{FDM} $ refers to the residual corresponding to a single instance of $ \mvec{S} $. So, to train the network against all the available data of $ \mvec{S} $, we define the following loss function:
\begin{align}\label{def:fdm-loss-stochastic-expectation}
	L_{FDM} = \mathbb{E}_{\omega\sim \Omega} \left\| \mvec{R}_{FDM}[\mvec{S}(\omega),\mvec{U}(\mvec{S}(\omega);\netparams)] \right\|^2_2.
\end{align}
To calculate the expectation numerically over the sample space $ \Omega $, we use a finite quasi-random sample sequence (such as Sobol sequences)  and define the approximate/numerical loss function as $ \hat{L}_{FDM} $:
\begin{align}\label{def:fdm-loss-stochastic-numerical}
	\hat{L}_{FDM}(\netparams) = \frac{1}{N_s} \sum_{i = 1}^{N_s}\left\| \mvec{R}_{FDM}[\mvec{S}(\omega_i),\mvec{U}(\mvec{S}(\omega_i);\netparams)] \right\|^2_2.
\end{align}

The loss function defined in \ref{def:fdm-loss-stochastic-numerical} evaluates the loss when the problem data $ s $ is a function of the random variable $ \omega $ and therefore the dataset $ \{S_i\}_{i = 1,..,N_s} $ is generated by constructing the sequence $ \{\omega_i\}_{i=1,..,N_s} $. But this loss function can also be used in the case when the dataset is not governed by a known probability distribution. In that case, we simply use:
\begin{align}
	\hat{L}_{FDM}(\netparams) = \frac{1}{N_s} \sum_{i = 1}^{N_s}\left\| \mvec{R}_{FDM}[\mvec{S}_i,\mvec{U}(\mvec{S}_i;\netparams)] \right\|^2_2.
\end{align}

The loss function $ \hat{L}_{FDM} $ is now a function of $ \mvec{\theta} $, and we can minimize $ \hat{L}_{FDM} $ with respect to $ \mvec{\theta} $ to reach the optimum network parameters,
\begin{align}
	\netparams^* = \arg\min_{\netparams} \hat{L}_{FDM}(\netparams).
\end{align}
% add comment about nonlinear equations

==> sections/formulations-fem-loss.tex <==
\subsubsection{Finite element based loss function}\label{sec:loss-fem}
The finite element based loss function is inspired by the Galerkin formulation of an elliptic PDE as well as the Rayleigh-Ritz method. In this case, we actually construct a function of certain regularity in the domain variable $ \xvec $, as opposed to just assuming a function of certain differentiability at the collocation points, as was the case in Sec. \ref{sec:loss-fdm}.

Suppose $ H^1(D) = W^{1,2}(D) $ denotes the Sobolev space of functions whose first derivatives are square integrable. Define the space $ V $ as
\begin{align}\label{eq:def:function-space-V}
	V = \setbuilder{v\in H^1(D) : v(0,y) = 1, v(1,y) = 0}.
\end{align}
Then the Galerkin formulation of equation \ref{eq:poisson-kl-intro} is to find $ u\in V $ such that,
\begin{align}\label{eq:galerkin-formulation-poisson-kl}
	B(u,v) = L(v) \ \ \forall v\in V,
\end{align}
where,
\begin{subequations}\label{eq:def:bilnear-linear-form}
	\begin{align}
		B(u,v) &= \int_{\spatialD}(\grad v\cdot \grad u) d\xvec \\
		L(v) &= \int_{\spatialD} vf d\xvec.
	\end{align}
\end{subequations}

Equation \ref{eq:galerkin-formulation-poisson-kl} yields an algebraic equation for each function $ v $ taken from the space V. Thus, if $ V $ is discretized such that it can be represented by a finite basis, then the Galerkin formulation \ref{eq:galerkin-formulation-poisson-kl} yields a finite system of algebraic equations.

From the principle of variational formulation, it is also known that equation \ref{eq:galerkin-formulation-poisson-kl} is the Euler-Lagrange equation of the following functional $ J(u) $ of $ u \in V $:
\begin{align} \label{eq:def:loss-functional-inner-product-form}
	J(u) = \half B(u,u) - L(u).
\end{align}
Therefore, the solution $ u $ can also be written as the minimizer of the cost function $ J $:
\begin{align}\label{eq:minimization-problem-continuous}
	u = \argmin_{u\in V} J(u).
\end{align}

In \diffnet, we make use of this functional $ J $, but instead of minimizing it against the solution $ u $, we minimize it against the network parameters $ \theta $. Since $ V $ is an infinite dimensional space, we need to discretize it to a finite subspace where we can evaluate $ J $. For this, let $ \mesh $ be a discretization of $ \spatialD $ into $ \nel $ ``finite'' elements $ K_i $ such that $ \cup_{\nel}K_i = D $. Then the discrete function space $ V^h $ is define as:
\begin{align}
	V^h = \setbuilder{v^h \in V: v^h|_{K}\in P_m(K), \ K\in \mesh},
\end{align}
where $ P_m(K) $ denotes the set of polynomial functions of degree $ m $ define on $ K $. Let the dimension of $ V^h $ be $ N $, which essentially means that the number of unknowns in the domain is also $ N $. Suppose $ \{ \phi_i(\xvec) \}_{i = 1}^{N} $ is a suitable basis that span $ V^h $. Then any function $ \uh \in V^h $ can be written as
\begin{align}\label{eq:def:fem-function-approximation-0}
	\uh(\xvec) = \sum_{i = 1}^{N} \phi_i(\mvec{x})U_i,
\end{align}
where $ U_i $ are the function values at the nodal points in the mesh $ \mesh $. 
Then equation \ref{eq:minimization-problem-continuous} can be rewritten for $ \uh $ as:
\begin{align}\label{eq:minimization-problem-discrete}
	\uh = \argmin_{\uh \in V^h} J(\uh).
\end{align}

A minimization problem such as \ref{eq:minimization-problem-discrete} is known as the Rayleigh-Ritz method. But in the presence of a neural network, we minimize $ J $ with respect to the network parameter $ \netparams $ instead of $ \uh $. For this, we need to first explicitly state the $ \theta $ dependence of $ \uh $. This can be done by a slight modification to \ref{eq:def:fem-function-approximation-0} as below:
%Equation \ref{eq:def:fem-function-approximation-0} still needs to be made precise about the dependence on the the network parameter $ \theta $ as well as the network input $ s $. As in the case of the finite difference based method, each $ U_i $ is a function of the network parameter $ \netparams $. So the precise notation for \ref{eq:def:fem-function-approximation-0} is
\begin{align}\label{eq:def:fem-function-approximation-1}
	\uh(\xvec;\netparams) = \sum_{i = 1}^{N} \phi_i(\mvec{x})U_i(\theta),
\end{align}
along with a generalization of the function space $ V $ as:
\begin{align}\label{eq:def:function-space-V-theta}
	\spaceVtheta = \setbuilder{v(\theta)\in H^1(\spatialD):v(x=0,y;\netparams) = 1, v(x=1,y;\netparams)=0}.
\end{align}
Then we can finally write down the \diffnet{} solution $ \uh_{\netparams^*} $ in two steps:
\begin{subequations}\label{eq:minimization-problem-theta-1}
	\begin{align}
		\netparams^* &= \argmin_{\netparams \in \Theta} J(\uh(\xvec; \netparams)) \\
		\uh_{\netparams^*} &=  \uh(\xvec; \netparams^*)
	\end{align}
\end{subequations}

The discussion leading to \ref{eq:minimization-problem-theta-1} is based on a non-parametric diffusivity, i.e., $ \tilde{\diffusivity} = \diffusivity(\xvec) $. When the diffusivity is parameterized by $ \omega $, i.e., $ \tilde{\diffusivity} = \diffusivity(\xvec,\omega) $, then the function space $ V^h(\netparams) $ needs to be modified as:
\begin{align}\label{eq:def:function-space-V-theta-stochastic}
	V^h_\netparams = \setbuilder{v: \| v(\xvec,\omega; \netparams) \|_{V^h_{\netparams}} < \infty,\ v(x=0,y,\omega;\netparams) = 1, v(x=1,y,\omega;\netparams)=0}
\end{align}
where, $\|\cdot\|_{V^h_{\netparams}}$ is the energy norm
\begin{align}\label{eq:def:stochastic-norm}
	\|v\|_{V^h_{\netparams}}^2 = \mathbb{E}_{\omega\sim\Omega}\left[\int_D \nu(\mvec{x}, \omega; \netparams)|\nabla v|^2d\mvec{x}\right].
\end{align}
With this choice of function space, the FEM loss function can be written as:
\begin{align}\label{def:fem-loss-stochastic-expectation}
	L_{FEM}(\netparams) = \mathbb{E}_{\omega\in\Omega}J(\uh(\xvec, \omega; \netparams))
\end{align}

The right hand side of \ref{def:fem-loss-stochastic-expectation} involves two integrations: one over the spatial domain $ \spatialD $ and the other an expectation over $ \Omega $. The integration over $ \spatialD $ is evaluated numerically using Gaussian quadratures rules. And the expectation over $ \Omega $ is evaluated approximately by a summation over a finite number of samples, similar to \ref{def:fdm-loss-stochastic-numerical}, i.e.,
\begin{align}\label{def:fem-loss-stochastic-numerical}
	\hat{L}_{FEM}(\netparams) = \frac{1}{N_s}\sum_{i = 1}^{N_s}J(s(\omega), \uh(\xvec,\omega); \theta).
\end{align}

The loss function $ \hat{L}_{FEM}(\netparams) $ is now just a function of $ \netparams $ and we can minimize it with respect to $ \netparams $, just as in the case of $ \hat{L}_{FDM}(\netparams) $,
\begin{subequations}\label{eq:minimization-problem-theta-2}
	\begin{align}
		\label{eq:minimization-problem-theta-2-opt}
		\netparams^* &= \argmin_{\netparams \in \Theta} \hat{L}_{FEM}(\netparams) \\
		\label{eq:minimization-problem-theta-2-sol}
		\uh_{\netparams^*} &=  \uh(\xvec, \omega; \netparams^*).
	\end{align}
\end{subequations}
%The FEM involves the weakening of the PDE using an appropriate weighting functions. As in the FDM case, we consider a discretization of the domain $ D $ into a finite number of non-overlapping elements denoted by $ Q_i $, $ i = 1,2,\ldots,\nel $ such that $ \cup_{i}^{nel} Q_i = D $. The unknown solution can be approximated as:
%
%where $\phi_i$ are the finite element basis functions.

%FEM is essentially an integrated method. Since $ \uh(\mvec{x}) $ is not a collection of values any more (unlike FDM), an integration needs to be carried out in order to get rid of the explicit dependence on $ \mvec{x} $. This fact also gives a very natural hint on how to define the loss function.

%\bk{can we be more certain than might be here?}In fact, there might be multiple ways to define the loss function using FEM approximation. We discuss two of them below:

% \begin{itemize}
% 	\item \textbf{Non-weighted loss}\bk{better to remove this}
% 	\begin{align}
% 	\mathcal{N}(u;s) -f = 0
% 	\end{align}
% 	\begin{align}
% 	R_{\theta} = \left\| \mathcal{N}(u_{\theta};s) -f \right\|^2 = \int_{D} \left[ \mathcal{N}(u_{\theta};s) -f \right]^2 d\mvec{x}
% 	\end{align}
% 	Associated optimization problem:
% 	\begin{align}
% 	\theta^{*} &= \argmin_{\theta} \left\| \mathcal{N}(u_{\theta};s) -f \right\|^2 \\
% 	u^{*} &= u_{\theta^*}
% 	\end{align}
% 	This loss function uses the strong form of the PDE as opposed to the weak form, thus the differentiability of the basis functions must be higher than the highest order appearing in the PDE. In this current paper, we do not pursue this approach.
	
%This approximation is plugged into the PDE, after which we invoke Galerkin's method. That is, multiply the PDE with a test function and reduce the differentiability requirement on $ u^h $ via integration by parts \footnote{For completeness, we assume $u^h_{\theta} \in V \subset H^1(D)$ where $ H^1(D) $ denotes the Hilbert space of functions on $ D $ that have square integrable first derivatives,}:
%\begin{align}
%\int_{\Omega} v\left[ \mathcal{N}(u^h_{\theta};s) -f \right] d\mvec{x} &= 0 \text{ }\forall v\in V
%\end{align}
%Which results in this following (standard FEM) form
%\begin{align}
%B(v,u^h_{\theta}) - L(v) &= 0\text{ }\forall v\in V
%\end{align}
%where $B(v,u^h_{\theta})$ is the bilinear form that encodes the PDE, while $L(v)$ is the linear form that encodes the load and boundary conditions. By choosing the test function to be the (unknown) solution, $u^h_{\theta}$, we get an energy functional 
%\begin{align}
%J(u^h_{\theta}) = \frac{1}{2} B(u^h_{\theta},u^h_{\theta}) - L(u^h_{\theta}),
%\end{align}
%whose minima is the sought solution $ u^h_{\netparams^*} $, where
%\begin{align}
%	\netparams^* = \arg\min_{\netparams} J(u^h_\netparams).
%\end{align}
% 	Associated optimization problem:
% 	\begin{align}\label{def:fem-weighted-optimization}
% 	\theta^{*} &= \argmin_{\theta} J(u_{\theta}) \\
% 	u^{*} &= u_{\theta^*}\label{def:u-optimal}
% 	\end{align}
%\end{itemize}
% \bk{need to define $B, L$}
% $ J(u,u) $ has the interpretation of the energy of the system, and the optimization problem is similar to the minimum energy principle, the only difference being that the minimization in ~\ref{def:fem-weighted-optimization} is with respect to $ \theta $ instead of $ u $. \ch{} \bg{To Review}
%This energy functional accounts for the PDE as well as all Neumann (and Robin) conditions. This serves as our loss function.
%\subsection{Non-weighted loss}
%\begin{align}
%\mathscr{L}(u) -f = 0
%\end{align}
%\begin{align}
%R_{\theta} = \left\| \mathscr{L}(u_{\theta}) -f \right\|^2 = \int_{\Omega} \left[ \mathscr{L}(u_{\theta}) -f \right]^2 d\mvec{x}
%\end{align}
%Associated optimization problem:
%\begin{align}
%\theta^{*} &= \argmin_{\theta} \left\| \mathscr{L}(u_{\theta}) -f \right\|^2 \\
%u^{*} &= u_{\theta^*}
%\end{align}
%
%\subsection{Weighted loss}
%\begin{align}
%\mathscr{L}(u) -f = 0
%\end{align}
%Assuming $u_{\theta} \in V$
%\begin{align}
%\int_{\Omega} v\left[ \mathscr{L}(u_{\theta}) -f \right] d\mvec{x} &= 0 \text{ }\forall v\in V\\
%B(v,u) - L(v) &= 0\text{ }\forall v\in V
%\end{align}
%The corresponding energy functional is 
%\begin{align}
%J(u) = \frac{1}{2} B(u,u) - L(u)
%\end{align}
%Associated optimization problem:
%\begin{align}
%\theta^{*} &= \argmin_{\theta} J(u_{\theta}) \\
%u^{*} &= u_{\theta^*}
%\end{align}
% \textbf{Note} We have used the superscript $ d $ in a loose sense, to denote a discrete quantity in both FDM and FEM context. So in FDM context $ U^d_\theta $ just means a vector such as $ \mvec{U} = (U_1,U_2,..,U_N) $, whereas in the FEM context $ U^d_\theta $ can mean both the discrete function $ u^h $ (as in Equation \ref{def:fem-function-approximation}) or the unknown coefficients (nodal values) $ \mvec{U} = (U_1,U_2,..,U_N) $

==> sections/implementations.tex <==
\section{Implementations}

%\input{figure_panels/derivative-calc-illustration-fdm.tex}
\input{figure_panels/derivative-calc-illustration-fem.tex}

\begin{figure}[!htb]
	\centering
	\includegraphics[width=0.99\linewidth]{images/UNetArch.png}
	\caption{UNet architecture used for training \invnet{}}
	\label{fig:unetarch}
\end{figure}

\subsection{Model architecture for \invnet{}}\label{sec:model-arch}
Due to the structured grid representation of $\mathcal{S}^d$ and similar structured representation of $U^d_\theta$, deep convolutional neural networks are a natural choice of network architecture. The spatial localization of convolutional neural networks helps in learning the interaction between the discrete points locally. Since, the network takes an input of a discrete grid representation (similar to an image, possibly with multiple channels) and predicts an output of the solution field of a discrete grid representation (similar to an image, possibly with multiple channels), this is considered to be similar to a image segmentation or image-to-image translation task in computer vision. U-Nets~\citep{ronneberger2015u,cciccek20163d} have been known to be effective for applications such as semantic segmentation and image reconstruction. Due to its success in diverse applications, we choose U-Net architecture for \invnet{}. The architecture of the network is shown in Figure~\ref{fig:unetarch}. First, a block of convolution, and instance normalization is applied. Then, the output is saved for later use during skip-connection. This intermediate output is then down sampled to a lower resolution for a subsequent block of convolution, instance normalization layers. This process is continued for two more times. Now, the upsampling starts where, the saved outputs of similar dimensions are concatenated with the output of upsampling for creating the skip-connections followed by a  convolution layer. LeakyReLU activation was used for all the intermediate layers. The final layer has a Sigmoid activation. 
% Next we explain the training procedure used for training \invnet{}.

\subsection{Applying boundary conditions}\label{sec:boundary-conditions}
In \invnet{}, the Dirichlet boundary conditions are applied exactly. The query result $ U^d_\theta $ from the network pertains only to the interior of the domain. The boundary conditions need to be taken into account separately. There are two ways of doing this:
\begin{itemize}
	\item Applying the boundary conditions exactly (this is possible only for Dirichlet conditions in FEM/FDM; and the zero-Neumann case in FEM)
	\item Taking the boundary conditions into account in the loss function, thereby applying them approximately.
\end{itemize}

We take the first approach of applying the Dirichlet conditions exactly (subject to the mesh). Since the network architecture is well suited for 2d and 3d matrices (which serve as adequate representation of discrete field in 2d/3d on regular geometry), the imposition of Dirichlet boundary conditions amounts to simply padding the matrix by the appropriate values. A zero-Neumann condition can be imposed by taking the ``edge values" of the interior and copying them as the padding.
A nonzero Neumann condition is slightly more involved in the FDM case since additional equations need to be constructed; but if using FEM loss, this can be done with another surface integration on the relevant boundary.

\subsection{Calculation of derivatives and integration}\label{sec:derivative-integal-calc-detail}
The derivatives in FDM are calculated by in-built convolution operations. \invnet{} takes an image representation of the input field and returns another image for the solution. Thus, the vector $ U^d_\theta $ is represented as a matrix (or image) in the code. There is an advantage of using this representation, which is that the derivative calculations can be made very fast using convolution operations. The stencil size determines the size of the kernel, and the FDM difference coefficients form the elements of the kernel. This convolution is only performed within the loss function, and thus has no relation to the convolutional neural network that is used to approximate the solution. See Figure ~\ref{fig:fdm-grid-example} and ~\ref{fig:fdm-5pt-laplacial-conv-example} for example.

The same goes for the integration process in FEM. The full domain integration (i.e., $ \int D $) is nothing but the simple sum of the integration over the individual elements (i.e., $ \sum_{i = 1}^{N_{el}} \int D_i $). This integration over an individual element is in turn the simple weighted sum of the integrand evaluated at the Gauss quadrature points. This evaluation at a single Gauss point can be represented as convolution. Thus, if there are 4 Gauss points in each element, then 4 convolution operations will evaluate the integrand at those points for each element. After that, we only need to sum across Gauss points first, then followed by a sum across elements. See Figure ~\ref{fig:fem-mesh-with-gauss-pt} and ~\ref{fig:fem-function-evaluation-at-single-gauss-pt} for example.


%$U^d_\theta$ is similarly the discrete (unknown) solution to the PDE. In case of FDM, $U^d_\theta$ would mean a collection of values $\underline{U}$; whereas, in case of FEM, ${U^d_\theta}$ will mean a linear combination of a finite number of polynomial functions. Here we use the superscript $ d $ to loosely denote a discrete quantity either in FDM or in FEM. But it should be kept in mind that in case of FDM, a quantity $ f^d $ is just a collection of real values $f^d_{FDM} = \underline{f} = (f_1,f_2,...,f_N)\in\mathbb{R}^{N} $, whereas when we say $ f^d $ in the FEM context, it really means a function in the form of $ f^d_{FEM} = f^h = \sum_{i = 1}^{N}N_i(\mvec{x})f_i : D\rightarrow \mathbb{R}$.



%\subsection{Linear Poisson equation in 2D}
%The Poisson equation is given by
%\begin{align}
%	\grad\cdot(\tilde{\nu}(\mvec{x})\grad u) &= 0 \text{  in  } D \\
%	u(0, y) &= 1 \\
%	u(1, y) &= 0 \\
%	\partialder{u}{n} &= 0 \text{ on other boundaries} 
%\end{align}
%
%The loss function:
%\begin{align}
%	R = \int \tilde{\nu}|\grad u|^2 d\mvec{x}
%\end{align}



%\subsection{Linear Heat equation in 1D+T}
%The linear heat equation is given by
%\begin{align}
%	\begin{cases}
%		u_t - \visco u_{xx} = f \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } \Gamma_s\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
%	\end{cases}
%\end{align}
%where $\visco = \visco (\underline{x},t)$ and the forcing $f = f(\underline{x},t)$.
%
%The loss function:
%\begin{align}
%	R_u = \int \left[uu_t + \visco \left( u_x \right)^2\right]dxdt
%\end{align}
%\begin{align}
%	R_{LS} &= \int \left(u_t - \visco u_{xx}\right)^2 dxdt \\
%	&= \int \left((u_t)^2 - 2\visco u_t u_{xx} + (\visco u_{xx})^2\right) dxdt \\
%	&= \int \left[(u_t)^2 + 2\visco u_x u_{xt}\right]dxdt
%\end{align}
%
%\begin{align}
%	R_{GLS} &= \int \left[uu_t + \visco \left( u_x \right)^2\right]dxdt + \int \tau u_t \left(u_t - \visco u_{xx}\right) dxdt \\
%	&= \int \left[uu_t + \visco \left( u_x \right)^2 + \tau (u_t)^2 + \tau \visco u_x u_{xt}\right]dxdt 
%\end{align}
%
%\subsection{Inviscid/Burgers equation in 1D+T}
%The Burgers' equation is given by
%\begin{align}
%	\begin{cases}
%		u_t + u u_x - \visco u_{xx} = f \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } \Gamma_s\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
%	\end{cases}
%\end{align}
%where $\visco = \visco (\underline{x},t)$ and the forcing $f = f(\underline{x},t)$.
%
%The FDM loss function:
%The FDM loss function:
%\begin{align}
%	R = \sum_{i}^{N_{xy}} \left\| \partialder{u^i}{t} + u^i\partialder{u^i}{x}\right\|^{2} + \sum_{i}^{N_{bn}}\gamma \left(\left\|u - u^b(\cdot, x_0)\right\|^2 + \left\|u - u^b(t_0,\cdot)\right\|^2\right)
%\end{align}
%
%\begin{equation}
%{\partial u \over \partial t} + u {\partial u \over \partial x} = 0
%\label{eq:Inviscid_Burgers}
%\end{equation}
%
%\begin{equation}
%u(x,t=0) = \frac{1}{2}(1 - cos(2\pi c x))
%\label{eq:initial-condition}
%\end{equation}
%where $c \ge 0$ is the parameter, and the domain of interest is the unit square, \newline
%$(x,t) \in \color{black}[0,1]\times[0,0.2]$.

%\subsection{First order wave equation}
%The wave equation is given by
%\begin{align}
%	\begin{cases}
%		\frac{\partial u}{\partial t} + a\frac{\partial u}{\partial x} = 0 \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } x=0\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0
%	\end{cases}
%\end{align}
%with $u_0(x) = e^{-\frac{(x-0.4)^2}{0.01}}$
%\begin{align}
%	R_{\theta} = \left\|\frac{\partial u}{\partial t} + a\frac{\partial u}{\partial x} \right\|^2
%\end{align}
%
%\subsection{Wave equation in 1D+T}
%The wave equation is given by
%\begin{align}
%	\begin{cases}
%		\frac{\partial^2 u}{\partial t^2} - c^2 \frac{\partial^2 u}{\partial x^2} = f \qquad &\text{in } \Omega = (0,1)\times(0,1]\\
%		u = 0 & \text{on } \Gamma_s\\
%		u = u_0(\mvec{x}) & \text{on } \Gamma_0\\
%		\partialder{u}{t} = v_0(\mvec{x}) & \text{on } \Gamma_0
%	\end{cases}
%\end{align}
%where $c$ is the wave velocity and the forcing $f = f(\underline{x},t)$.

==> sections/intro.tex <==
%\section{Reference Notes (will be deleted)}
%	
%	Solving PDEs with a neural network as an approximation, a priori fixed mesh - (\cite{lee1990neural,lagaris1998artificial,lagaris2000neural,malek2006numerical,rudd2015constrained})
%	
%	PINN - (\cite{raissi2018hidden,raissi2019physics,kharazmi2019variational})
%	
%	Data-Driven Identification of Parametric Partial Differential Equations - (\cite{rudy2019data})
%	
%	Data driven Eulerian - (\cite{tompson2017accelerating})
%	
%	Optimal weighting of PDE loss and BC loss - (\cite{van2020optimally})
%	
%	DGM, was published at the same time as PINN, but arguably received much lesser limelight (\cite{sirignano2018dgm})
%	
%	Full field solutions - (\cite{paganini2018calogan,botelho2020deep,zhu2019physics})
%	
%	Pointwise predictions - (\cite{yang2018physics,pang2019fpinns,karumuri2020simulator,han2018solving,michoski2019solving})
%	
%	General class of pdes - (\cite{zhu2019physics,sirignano2018dgm,yang2018physics})
%	
%	Improvement in numerical linear algebra and single instance of pde: (\cite{pang2019fpinns,karumuri2020simulator,hsieh2019learning,katrutsa2017deep,greenfeld2019learning})
%	
%	Variational energy based: (\cite{samaniego2020energy})
%	
%	%	In many science and engineering disciplines, solving partial differential equations has long 

\section{Introduction}
\begin{figure}[t!]
	\begin{tikzpicture}
	\draw (0, 0) node[inner sep=0] {\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{images/invnet-schematic.png}};
	\draw (-2.9, -1.8) node {$S^d$};
	\draw (2.9, -1.8) node {$U^d$};
	\draw (0.2, -1.8) node {$G_{nn}$};
	\draw (0.2, -2.5) node {(a)};
	\end{tikzpicture}\hfill
	% 	\label{fig:invnet-network-representation}
	% \end{figure}
	% 	\begin{figure}
	\begin{tikzpicture}
	\draw (0, 0) node[inner sep=0] {\includegraphics[trim=0 0 0 0,clip,width=0.45\linewidth]{images/pinn-schematic.png}};
	\draw (-3.0, -0.3) node {$\mvec{x}_i$};
	\draw (1.3, 0.4) node {$u_{i}$};
	\draw (4.0, -0.4) node {$\mathbb{R}$};
	\draw (1.8, -1.15) node {$a$};
	\draw (3.3, -1.1) node {$b$};
	\draw (0.2, -1.8) node {$G_{nn}$};
	\draw (0.2, -2.5) node {(b)};
	\end{tikzpicture}
	\caption{(a) In our \invnet{} approach, we train a neural network to produce a discretized field solution over a mesh. Such an approach offers a direct link to powerful PDE analysis techniques, at the cost of a larger network. (b) In contrast, neural methods (like \cite{lagaris1998artificial,raissi2019physics}) are trained to produce point predictions: $ \neuralMap : D\rightarrow \mathbb{R}$, which are easier to train, but more difficult to analyze.} 
	\label{fig:common-networks-for-pdesolve}
\end{figure}

Numerical methods -- finite difference methods (FDM), finite element methods (FEM), spectral methods -- for solving PDEs discretize the physical domain (into cells, elements, ect) and \textit{approximate} the solution over this discretized domain using select families of basis functions \cite{hughes2012finite,leveque2007finite,trefethen2000spectral}. There is well developed and elegant theory that connects the discretization of the domain (in terms of element/cell dimension, $h$) and the properties of the basis functions (in terms of polynomial order, $\alpha$) with the quality of the ensuing numerical solution to the PDE. In particular, numerical stability arguments and \textit{a priori} error estimates allow users to judiciously reason about accuracy, robustness, and convergence \cite{brenner2007mathematical,larson2013finite}. Such theoretical arguments rely on the spatial discretization of the domain, and properties of the basis functions. Here, we formulate loss functions and networks that produce field solutions of PDEs (\figref{fig:common-networks-for-pdesolve}(a))  -- to be analogous with numerical PDE solvers --  in contrast to current neural PDE solvers that predominantly produce point estimate (\figref{fig:common-networks-for-pdesolve}(b)). %The guiding principle opens up theoretical arguments f. 

%The common theme that runs through all these methods is the idea that, even if an exact infinite dimensional solution is practically unobtainable (except for some trivial problems), it is still possible to obtain a \textit{finite dimensional} solution that is ``close enough" to the exact one. But this goal of rendering the finite dimensional problem, also known as ``discretization", is achieved through different devices in all these methods, as can be guessed from their naming. FDM does this by discretizing the domain of the PDE into finite number of points; and then assuming the existence of certain derivatives on the exact solution, it then attempts to obtain the numerical values of the function corresponding to those discrete points of the domain. On the other hand, FEM takes a completely different route where not only the domain is discretized, but also the solution is represented as a linear combination of a finite number of piecewise basis functions. 	An important characteristic of such approaches is that the methods are designed by keeping in mind the topology of the domain. Locality of information is replicated through the discrete points. This is because, although the exact solution is a function of a continuous variable, the discrete solution is determined by its values at discrete points, which often interact locally. 
% But with the development of deep neural networks and the prolific success in adapting deep learning methods into many diverse problems, attempts have been made to apply deep learning methods to solve PDEs. Some of the early works in this direction attempted to solve ODEs using a neural network but mostly focused on the linear algebra aspect of the network, i.e., with an eye to leverage the optimization formulation available with such a neural network \cite{lee1990neural}. The idea of using using a feed forward network to obtain a mapping between the domain variable (say, $ \mvec{x} $) and the range variable (say, $ u $) followed very soon \cite{lagaris1998artificial,lagaris2000neural}. $ u $ was considered as comprising of two components, the ``interior" and the ``boundary" parts. Only ``interior" part was for the network to learn, whereas the ``boundary" part was chosen to satisfy the applied boundary conditions. Much deeper network has also been used, particularly to solve higher order ODEs and system of ODEs \cite{malek2006numerical,rudd2015constrained}.


In recent years data-driven \cite{rudy2019data,tompson2017accelerating} and data-free approaches \cite{raissi2019physics,kharazmi2019variational,sirignano2018dgm,yang2018physics,pang2019fpinns,karumuri2020simulator,han2018solving,michoski2019solving,samaniego2020energy} for solving PDEs have been proposed. Most of these models are designed for pointwise prediction, i.e., the networks in these cases simply take as input $ \mvec{x} $ and produces an output value of $ u $, thereby calculating the value of $ u $ at one particular point. Some of these methods satisfy/apply the boundary conditions exactly \cite{lee1990neural,lagaris1998artificial,malek2006numerical} and others do that in an approximate manner \cite{lagaris2000neural,raissi2019physics,sirignano2018dgm}. Many of these methods do not require a mesh, and thus rely on collocating points from the domain randomly. The methods that approximately satisfies the boundary conditions do so by adding a loss function with respect to the specified boundary conditions. It has been shown by \cite{van2020optimally,wang2020understanding} that these losses have to be carefully weighted, making this an non-trivial exercise in hyper parameter tuning. This underlines the difficulty of applying the boundary conditions in a neural network-based method (or simply neural method).

 %There has also been efforts at improving the numerical linear algebra aspect of a neural network tasked with the job of finding an approximate solution to a PDE.

 %So in essence, the modern neural methods take the view that a deep neural network can represent complicated functions, and thus attempt to approximate the solution of the PDE through the neural network. In a way this seems an improvement over the classical numerical methods, in that the discrete solution is approximated through a highly complicated and nonlinear mapping as opposed to a linear combination of local functions of limited differentiability (which may not be the case for the exact solution). But on the other hand, these neural methods do not take into account the domain topology, and thus the ``local'' nature of the solution and sparsity of matrices that comes naturally to the classical methods, is missing in the neural methods. In addition, imposition of boundary conditions can be difficult in neural methods.
 

\textbf{Contributions:} We build upon some recent efforts that train networks to predict the full-field solution \cite{paganini2018calogan,botelho2020deep,zhu2019physics}. The specific contributions of this paper are :
\begin{enumerate}
	\item We present an algorithm that is bridges traditional numerical methods with neural methods. The neural network is designed to map inputs to the discretized field solution $ u $. However, the neural network is \textit{not responsible} for ensuring the spatial differentiability of the solution. Rather, the discrete field solution relies on traditional numerical methods (and associated numerical differentiation and quadrature) for construction of the loss function. Such an approach allows natural incorporation of different boundary conditions, and allows \textit{a priori} error estimates.
    \item We define two loss functions based on FDM and FEM. By setting up the loss function this way, we create the function space with appropriate differentiability and also account for the ``local'' nature of the solution. 
    \item We demonstrate \invnet{}'s performance on linear Poisson equation in 2D and steady heat transfer.
\end{enumerate}
%  \item Using these two loss functions we develop a neural approximation framework, \invnet{}, for providing learning of the mapping for parametric PDEs.


==> sections/methods.tex <==
\section{Formulations}\label{sec:formulations}
\subsection{Neural approximation of the solution}\label{sec:neural-approximation-of-solution}
Instead of seeking a mapping between the domain and an interval on the real line (Fig.~\ref{fig:common-networks-for-pdesolve}(b)), we seek a mapping between the input $ s $ and the full field solution $ u $ in the discrete spaces (Fig.~\ref{fig:common-networks-for-pdesolve}(a)). $S^d$ denotes the discrete representation of the known quantity $s$. $S^d$ could be either available only at discrete points (perhaps from some experimental data); or in many cases, $s$ might be known in a functional form and thus $S^d$ will be simply the values of $s$  evaluated on the discrete points. Therefore, if we denote a \invnet{} (see Figure ~\ref{fig:common-networks-for-pdesolve}(a)) network by $ \neuralMap $, then $ \neuralMap $ takes as input a discrete or functional representation of $ s $ and outputs a discrete solution field $U^d_\theta$, where $\netparams$ denote the network parameters:
\begin{align}\label{def:neural-function-definition}
	U^d_\netparams = \neuralMap(S^d; \netparams)
\end{align}
%For example, if we consider a PDE defined on a 2D bounded domain, then $ \neuralMap $ simply takes a 2D matrix containing the values of $ s $ and returns the solution $ U^d_\theta $ which is also a 2D matrix.

An untrained network, as expected, will produce a mapping that does not satisfy the discrete PDE; in fact, it will show a huge error. Our goal is to bring this error down to an acceptable level, and thereby reaching a solution that is ``close enough" to the exact solution. And we do this by designing the loss function based on major ideas taken from the classical numerical methods. This is explained next.



\subsection{Loss functions inspired by numerical methods}\label{sec:loss-functions}
The design of the loss function, along with the choice of the neural mapping, forms the central part of our approach. As referenced before, the loss functions are based either on finite difference or on finite element discretization. We discuss both of these separately below.

%\input{sections/formulations-fdm-loss.tex}
\input{sections/formulations-fem-loss.tex}

\subsection{Training algorithm for \invnet{}}\label{sec:training-process}
We provide two versions of the training algorithm. (i) an algorithm for computing the solution for an instance of a PDE and (ii) an algorithm for approximating the solution for a parametric PDE. The model architecture and the loss function remain the same for both. For solution for an instance, we use a simple approach as explained in Algorithm~\ref{alg:pde-instance}. While sampling from a distribution of coefficients/forcing field for a parametric PDE, we employ the mini-batch based optimization approach as explained in Algorithm~\ref{alg:pde-parametric}. The sampling of the known quantities is performed by using Sobol sampling methodology. For training the neural network, we predict the solution field using sampled inputs and compute the loss using the FDM/FEM loss. We employ Adam optimizer with a learning rate of $1E-5$ for performing the optimization of the neural network parameters, $\theta$ using the gradients obtained from the FDM/FEM loss. 


%\begin{algorithm}[t]
%	\caption{Algorithm for an instance of a PDE}\label{alg:pde-instance}
%	\footnotesize
%	\begin{algorithmic}[1]
%		\STATE Initialize $ \neuralMap $, \textsc{tol}
%		
%		\FOR{\texttt{epoch} $ \leftarrow $ 1 to \texttt{max\_epoch}}
%		\STATE $U^d_\theta_{int} \gets G_{nn}(S^d)$ 
%		\COMMENT{``int" stands for interior nodes}
%		\STATE $U^d_\theta \gets U^d_\theta_{int}\chi_{int} + U^d_\theta_{bc}\chi_{b}$
%		\STATE $ L =  $
%		\ENDFOR 
%	\end{algorithmic}
%\end{algorithm}

\begin{algorithm}[t]
	\caption{Algorithm for an instance of a PDE}\label{alg:pde-instance}
	\begin{algorithmic}[1]
		\Require $ S^d $, $ (U^d_\theta)_{bc} $, $ \alpha $ and \textsc{tol}
		\State Initialize $ \neuralMap $		
		\For{\texttt{epoch} $ \leftarrow $ 1 to \texttt{max\_epoch}}
		\State $(U^d_\theta)_{int} \gets G_{nn}(S^d)$ 
		\Comment{``int" stands for interior nodes}
		\State $(U^d_\theta) \gets (U^d_\theta)_{int}\chi_{int} + (U^d_\theta)_{bc}\chi_{b}$
		\State  $loss = L(U^d_\theta)  $
		\State $ \theta \gets optimizer(\theta,\alpha,\grad_\theta(loss))$
		\EndFor		 		
	\end{algorithmic}
\end{algorithm}
\begin{algorithm}[t]
	\caption{Algorithm for parametric PDE}\label{alg:pde-parametric}
	\begin{algorithmic}[1]
		\Require $ S^d $, $ (U^d_\theta)_{bc} $, $ \alpha $ and \textsc{tol}
		\State Initialize $ \neuralMap $		
		\For{\texttt{epoch} $ \leftarrow $ 1 to \texttt{max\_epoch}}
		\For{\texttt{mb} $ \leftarrow $ 1 to \texttt{max\_mini\_batches}}
		\State Sample $S^d_{mb}$ from the set\\
		\State $(U^d_\theta)_{int,mb} \gets G_{nn}(S^d_{mb})$\\
		\Comment{``int" stands for interior nodes}
		\State $(U^d_\theta)_{mb} \gets (U^d_\theta)_{int,mb}\chi_{int} + (U^d_\theta)_{bc}\chi_{b}$
		\State  $loss_{mb} = L(U^d_\theta)  $
		\State $ \theta \gets optimizer(\theta,\alpha,\grad_\theta(loss_{mb})) $
		\EndFor
		\EndFor
	\end{algorithmic}
\end{algorithm}

==> sections/preliminaries.tex <==
\section{Mathematical Preliminaries}\label{sec:preliminaries}
Consider a bounded open (spatial) domain $D \in \mathbb{R}^n, n\geq 2$ with a Lipschitz continuous boundary $\Gamma = \partial D$. We will denote the domain variable as $\mvec{x}$, where the boldface denotes a vector or tuple of real numbers. In $ \mathbb{R}^n $, we have $ \mvec{x} = (x_1,x_2,\ldots,x_n) $; but for 2D and 3D domains, we will use the more common notation $ \mvec{x} = (x,y) $ and $ \mvec{x} = (x,y,z) $ respectively. Consider also a probability space $ (\Omega, F, P) $, where $ \Omega $ is the sample space, $ F $ is the $ \sigma $-algebra of the subsets of $ \Omega $ and $ P $, a probability measure.

On this domain $ D $, we consider an abstract PDE on the function $u: D\times \Omega \rightarrow \mathbb{R}$ as:

\begin{subequations}\label{pde:abstract-representation-continuous}
	\begin{align}
	\mathcal{N}[u; s(\mvec{x},\omega)] &=f(\mvec{x}),\quad \mvec{x}\in D,\ \omega\in\Omega \label{pde:abstract-equation}\\
	\mathcal{B}[u]&=g(\mvec{x}),\quad \mvec{x}\in\Gamma. \label{pde:abstract-bc}
	\end{align}
\end{subequations}
Here, $\mathcal{N}$ is a differential operator (possibly nonlinear) operating on a function $u$. The differential equation also depends on the data of the problem $s$ which in turn is a function of the domain variable $ \mvec{x} $ and parameter $ \omega $. Thus $ \mathcal{N} $ is essentially a family of PDE's parameterized by $ \omega $. $ \mathcal{B} $ is a boundary operator on $ u $. In general, there can be multiple boundary operators for different part of the boundary $ \Gamma $.

Given a PDE along with some boundary conditions, such as one presented in \ref{pde:abstract-representation-continuous}, the goal is to find a solution $ u $ that satisfies \ref{pde:abstract-representation-continuous} as accurately as possible. Previous works such as \cite{lagaris1998artificial,raissi2019physics,sirignano2018dgm} seek to find this exact mapping $u: D \rightarrow \mathbb{R}$. But as we present in the next section, we do not have to restrict ourselves to this mapping, and in fact, with the help of deep neural networks coupled with numerical methods, we can find other mappings to retrieve a discrete solution.

In this work, we will focus on the Poisson's equation with both Dirichlet and Neumann conditions applied on the boundaries, along with a heterogeneous and stochastic diffusivity:
\begin{align}\label{eq:poisson-pde}
	-\grad\cdot(\diffusivity(\mvec{x},\omega)\grad u) &= f(\mvec{x}) \text{  in  } D
\end{align}
along with the boundary conditions
\begin{align}
	u &= g \text{ on } {\Gamma_D}\label{eq:poisson-bc-dirichlet} \\
	\partialder{u}{n} &= h  \text{ on } {\Gamma_N} \label{eq:poisson-bc-neumann}
\end{align}
where $ \diffusivity $ is the \emph{permeability} (or \emph{diffusivity}) which depends on both $ \xvec $ and the random variable $ \omega $; and $ f $ is the forcing. In relation to Eq. \ref{pde:abstract-representation-continuous}, $ \diffusivity $ plays the role of the data $ s $. $ \Gamma_D $ and $ \Gamma_N $ are the boundaries of the domain $ D $ where Dirichlet and Neumann conditions are specified respectively. We will assume that $ \partial D = \Gamma = \Gamma_D \cup \Gamma_N$.

\subsection{Poisson's equation in heterogeneous media}\label{sec:poisson-kl-problem-intro}
We are mostly interested in the problem of a steady state mass (or heat) transfer through an inhomogeneous medium (material). This essentially means that the material has different properties at different points. The only material property appearing in the Poisson's equation (\ref{eq:poisson-pde}) is $ \nu(\mvec{x}) $, thus the inhomogeneity can be modeled by a spatially varying $ \nu $, i.e., $ \nu = \nu(\mvec{x}) $. The equation and the BC's are given by:
\begin{subequations}\label{eq:poisson-kl-intro}
	\begin{align}
		-\grad\cdot(\tilde{\nu}(\mvec{x})\grad u) &= 0 \text{  in  } D \\
		u(0, y) &= 1 \\
		u(1, y) &= 0 \\
		\partialder{u}{y}(x,0) &= 0 \\
		\partialder{u}{y}(x,1) &= 0
	\end{align}
\end{subequations}
where $ D $ is a hypercube domain in $ \mathbb{R}^n $, $ n = 2,3 $. The diffusivity/permeability $ \tilde{\diffusivity} $ is heterogeneous with respect to $ \xvec $ and is also parameterized by $ \omega\in\Omega $. The specific form of $ \tilde{\diffusivity} $ is given in \ref{def:poisson-nu-harmonic-expansion}. The stochastic description of $ \tilde{\diffusivity} $ is discussed below.



==> sections/results.tex <==
\section{Results}\label{sec:results}
%We present results from a canonical PDE in two and three dimensions. Specifically, we consider the Poisson equation.
%Numerical examples in this work are as follows:
%\begin{itemize}
%	\item Linear/Nonlinear Poisson (log permeability)	
%	\item Linear Heat equation in space-time
%	\item Inviscid/Viscid Burgers in space-time
%	\item Wave equation in space-time
%\end{itemize}

\subsection{Error convergence for a non-parametric Poisson problem} \label{sec:linear-poisson-manufactured}
At the outset, we want to validate the error bounds stated in section \ref{sec:errors}. To this end, we solve the following non-parametric Poisson's equation:
\begin{subequations}\label{eq:poisson-manufactured-pde}
	\begin{align}
	-\laplacian u &= f \ \ \text{in} \ \spatialD \subset \mathbb{R}^2 \\
	u &= 0 \ \ \text{on} \ \partial\spatialD,
	\end{align}
\end{subequations}
where $ D = [0,1]^2 $ is a two-dimensional square domain. The forcing is chosen as
\begin{align} \label{eq:poisson-mms-forcing}
	f = f(\mvec{x}) = f(x,y) = 2\pi^2\sin(\pi x) \sin(\pi y).
\end{align}
The exact solution to problem \ref{eq:poisson-manufactured-pde} with forcing \ref{eq:poisson-mms-forcing} is given by $ u_{ex}(x,y) = \sin(\pi x) \sin(\pi y) $. For solving this problem, we seek to train a \diffnet{} that can predict the solution $ u $ given the forcing $ f $. At the discrete level, the network takes input $ F^d $ and outputs $ U^d $. The loss function \ref{eq:def:loss-functional-inner-product-form} takes the concrete form:
% FDM based loss:
%\begin{align}\label{def:loss-fdm-poisson-manufactured}
%R = \sum_{i}^{N_{xy}} \| \grad\cdot[{\nu}(\mvec{x}^i]\grad u(\mvec{x}^i)) + f(\mvec{x}^i)\|^{2}
%\end{align}
\begin{align}\label{def:loss-fem-poisson-manufactured}
J(u) = \frac{1}{2} \int |\grad u|^2 d\mvec{x} - \int u f d\mvec{x}.
\end{align}
Fig. \ref{fig:poisson-manufactured-contours} shows the contours of the network input $ F^d $, output $ U^d $, the exact solution evaluated on the mesh $ \mesh $ (a $ 256\times 256 $ grid) and the error ($ U^d - U_{ex} $).
%\begin{figure*}[!htb]
%	\centering
%	%	\includegraphics[trim=100 0 619 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
%	\includegraphics[trim=150 5 100 10,clip,width=0.95\linewidth]{results_data/poisson-convergence/query_contour_0.png}
%	\caption{Solution to the linear Poisson's equation with forcing. From left to right: $f$, $u^h_\theta$, $u_{num}$ and ($u^h_\theta-u_{num}$). Here $u_{num}$ is a conventional numerical solution obtained through FEM. Diffusivity $\visco = 1$}
%	\label{fig:poisson-manufactured-contours-0}
%\end{figure*}
\begin{figure}[!htb]
	\centering
	\begin{minipage}{.7\textwidth}
		\centering
		\begin{tikzpicture}
		\begin{axis}[
		width=0.99\linewidth, % Scale the plot to \linewidth
		height=6cm,
		%grid=major, % Display a grid
		%grid style={line width=.1pt, draw=gray!50}, % Set the style
		xlabel={{\# step}}, % Set the labels
		ylabel={$\log_{10}(L)$},
		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
		x tick label style={rotate=0,anchor=north} % Display labels sideways
		]
%		\addplot+ [thick, mark=none] table[x expr={\thisrow{Step}},y expr={ln(\thisrow{Value})/ln(10)},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/run-version_5-tag-PDE_loss.csv};
		\addplot+ [thick, mark=none]
		table[x expr={\thisrow{Step}},y expr={ln(\thisrow{Value})/ln(10)},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/run-version_0-tag-PDE_loss.csv};
		\legend{$L_{FEM}$}
		\end{axis}
		\end{tikzpicture}
	\end{minipage}
	\caption{Loss \textit{vs} optimization steps for the losses \ref{def:loss-fdm-poisson-kl} and \ref{def:loss-fem-poisson-kl}}
\end{figure}
\begin{figure}[!htb]
	\centering
	%	\includegraphics[trim=100 0 619 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
	\includegraphics[trim=75 0 75 0,clip,width=0.95\linewidth]{results_data/poisson-convergence/mms-vis.png}
	\caption{Solution to the problem \ref{eq:poisson-manufactured-pde} with forcing \ref{eq:poisson-mms-forcing} on a $ 256\times 256  $ grid. (Left) the discrete forcing $ F^d $, (middle-left) the solution $ U^d $ obtained from a \diffnet{} with a U-net architecture, (middle-right) the exact solution $ u_{ex} = \sin(\pi x)\sin(\pi y) $ evaluated on the mesh, denoted $ U_{ex}^d $, (right) the error $ (U^d - U^d_{ex}) $.  From left to right: $f$, $u^h_\theta$, $u_{num}$ and ($u^h_\theta-u_{num}$). Note: $ \norm{u} = 0.499979 $, $ \norm{u_{ex}} = 0.5 $, $ \norm{u-u_{ex}} = 2.4\times 10^{-5} $.}
	\label{fig:poisson-manufactured-contours}
\end{figure}

To study convergence behavior, we repeat this procedure with varying mesh length $ h $, starting from $ h = \oneOver{8} $ and gradually decreasing $ h $ till $ h = \oneOver{256} $. The calculated errors for each resolution are reported in Fig. \ref{fig:convergence-plot-non-parametric}. 

Theorem \ref{thm:diffnet-errors-non-parametric} estimates the total error by the contributions from three individual sources of errors, namely, the error due to finite element discretization ($ \eDis $), the error due to network approximation capacity ($ \eCap $) and the error due to the optimization process ($ \eOpt $). Of these three error sources, $ \eDis $ maintains a particular relation to the discretization parameter $ h $ (i.e., the mesh size). The other two errors do not hold a straight-forward relation with the mesh size or the network parameters. Thus, we put the estimate \ref{eq:error-bound-non-parametric} to test by keeping both $ \eCap $ and $ \eOpt $ sufficiently low, so that the dominating error is the discretization error $ \eDis $.

\input{figure_panels/mms_conv.tex}

We illustrate this by running two sets of \diffnet{} simulations.
\begin{itemize}
	\item The first set is where we completely remove the neural network and optimize the loss directly with respect to the displacement variables $ \mvec{U}^h $, i.e.
	\begin{align}
		\uh = \argmin_{\uh \in \spaceVh} J(\uh),
	\end{align}
	which is nothing but a classic Rayleigh-Ritz optimization. The absence of a neural network eliminates the error $ \eCap $. So the total error is a combination of only $ \eDis $ and $ \eOpt $. The total errors from this algorithm are plotted against the mesh size  $ h $ in Fig. \ref{fig:convergence-plot-non-parametric} under the legend ``\diffnet{} (No network)''. We see that the error plot has a slope of 2.
		
	\item The second set uses a neural network. Thus the optimization statement is the same as presented in equation \ref{eq:minimization-problem-theta-2}. Therefore, as discussed in theorem \ref{thm:diffnet-errors-non-parametric}, the total error is a combination of all three errors indicated in. To illustrate the interplay between the individual components of errors in this case, the following two simple experiments were done:
	\begin{itemize}
		\item \textit{Keeping the network unchanged across all $ h $-levels}: If we choose a particular network and use it to solve equation \ref{eq:poisson-manufactured-pde}, then the errors do not necessarily decrease with a decrease in $ h $. As shown in Fig. \ref{fig:convergence-plot-non-parametric}, the errors actually increase when $ h>2^{-5} $. This reason for this behaviour is that, when $ h $ becomes low, the number of discrete unknowns in the mesh (i.e., $ U_i $'s in equation \ref{eq:def:fem-function-approximation-0}) increases. In fact, in this case, the number of basis functions / unknowns, $ N $  is exactly equal to $ \oneOver{h^2} $. As $ h $ decreases, the size of the output $ U_i $'s increase. But since the network remains the same, the discrete function space $ \spaceVh $ does not remain a subspace of $ \spaceVhtheta $ anymore. This network function class also needs to get bigger to accommodate all the possible functions at the lower values of $ h $. 
		\item \textit{Enhancing the network capacity with decreasing $ h $}: In the sister experiment, we increase the depth of the UNet, thereby increasing the capacity of the network, thus at every $ h $-level, the space $ \spaceVhtheta $ is large enough so that it is a superset of $ \spaceVh $. Our goal in this experiment is not to obtain the optimum superset of $ \spaceVh $, rather, we just look for one such superset $ \spaceVhtheta \supset \spaceVh $. The plot from this experiment shows a slope of 2, which means that both $ \eCap \approx 0 $ and $ \eOpt \approx 0 $, and the only dominant error is the discretization error $ \eDis $. The fact that $ \eOpt $ is negligible affirms that the optimization algorithm is able to find the correct optima within the function space.
	\end{itemize}
\end{itemize}
Fig. \ref{fig:convergence-plot-non-parametric} also shows a plot of errors obtained from solving the same problem using a conventional FEM code (using numerical linear algebra) for reference.

\subsection{Poisson's equation with parametric log permeability}\label{sec:results-poisson-kl-problem}
Our second illustration is the solution of the PDE defined in Sec \ref{sec:poisson-kl-problem-intro} (equation \ref{eq:poisson-kl-intro}), which is frequently used for simulating practical problems such as heat or mass transfer through an inhomogeneous media. We solve this problem in both 2D and 3D domains, i.e., $ D=[0,1]^2 $ as well as $ D=[0,1]^3 $; $ \tilde{\nu} $ is now a function of $ \mvec{x} = (x,y) $ and is also parametric, as mentioned in \ref{def:poisson-nu-harmonic-expansion}.

We seek a mapping of the form $ u = \neuralMap(\diffusivity) $, where $ \neuralMap $ denotes the neural network. So $ S^d $ refers to the discrete version of $ \diffusivity $. Following the principle of Karhunen-Loeve expansion as described in Sec. \ref{sec:poisson-kl-problem-intro}, the infinite dimensional random space is truncated into a finite dimensional space. Thereafter, a finite set of samples are prepared from this space for the training process. Suppose the number of samples is $ N_s $. Then the loss function takes the concrete form:
%\textbf{Note:} When the diffusivity is constant, the mapping between the forcing and the solution is linear (the previous example).  But the mapping between $ u $ and $\tilde{\nu} $ is not linear. This can also be seen since $ \tilde{\nu}  $ and $ u $ are multiplied together in the PDE.
%The loss function takes the concrete form:
%\begin{align}\label{def:loss-fdm-poisson-kl}
%R = \sum_{i}^{N_{xy}} \left\| \grad\cdot({\nu}(\mvec{x}^i)\grad u (\mvec{x}^i)) - f(\mvec{x}^i)\right\|^{2} 
%%+ \sum_{i}^{N_{bn}}\gamma \left\|\partialder{u}{n}\right\|^2
%\end{align}
\begin{align}\label{def:loss-fem-poisson-kl-concrete}
J = \oneOver{N_s} \sum_{i = 1}^{N_s} \int_{\spatialD} \tilde{\nu}_i(\xvec)|\grad u_i(\xvec)|^2 d\mvec{x},
\end{align}
where, $ u_i = \neuralMap(\diffusivity_i, \netparams) $.
Both Dirichlet and Neumann conditions are present in this equation. In \diffnet{}, the Dirichlet conditions are applied exactly. The zero-Neumann condition is also applied exactly at the continuous level, since the boundary integrals vanish at the continuous level (see equation \ref{eq:def:bilnear-linear-form}).

By optimizing the loss \ref{def:loss-fem-poisson-kl-concrete} as described in \ref{eq:minimization-problem-theta-2}, we attempt to  learn the distribution of the stochastic solution, given that the coefficients in the log permeability K-L sum come from a known range of values that depends on the parameter space $ \omega $. We truncate the K-L sum after 6 terms. These six coefficients form a six-dimensional space from which the coefficient tuples $ \{a_i\}_{i=1}^{6} $ can be drawn. The \diffnet{} is trained by selecting a finite number ($ N_s $) of pseudo-random samples from this 6-dimensional space. For the results shown below, we have taken $ N_s=65536 $. We used the Adam optimization algorithm, with a learning rate of $ 10^{-4} $. Once the network is trained, we can perform inference by evaluating the network mapping for any diffusivity $ \diffusivity $ taken from the sample space. To illustrate the nature of the input ($ \diffusivity $ or $ S^d $) and the solution ($ u $ or $ U^d $), we present an anecdotal (i.e., a non-special and random) set of $ S^d $ and $ U^d $ in Fig. \ref{fig:poisson-kl-contours-2}. A reference solution using a conventional FEM program is also presented therein. Furthermore, sectional line cuts for these contours are shown in Figure \ref{fig:line-cuts-kl-2d-single}. The line cuts display a close match between \diffnet{} and the numerical reference solution.
\begin{figure}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/g_inp_contour.png}}
	\end{minipage}
	%	\begin{minipage}{.24\textwidth}
	%		\centering
	%		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
	%		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/fdm/u_gen_contour.png}}
	%	\end{minipage}	
	\begin{minipage}{.32\textwidth}
		\centering
		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/fem/u_gen_contour.png}}
	\end{minipage}
	\begin{minipage}{.32\textwidth}
		\centering
		%	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/run_003-fem-sobol-query/query_contour_14.png}\\
		{\includegraphics[trim=400 200 450 190,clip,width=0.9\linewidth]{results_data//steady-heat-kl/sample-1/num/u_num.png}}
	\end{minipage}	
	\caption{(Left) contours of $ \nu $ corresponding to $ \underline{\omega} = (-1,2,1.5,-1.3) $, (middle) \diffnet{} with an FEM based loss, (right) reference numerical solution using FEM}
	\label{fig:poisson-kl-contours-2}
\end{figure}
\input{figure_panels/kl_line_cuts_2d.tex}
%\begin{figure}
%	\centering
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		width=0.99\linewidth, % Scale the plot to \linewidth
%		%height=6cm,
%		%grid=major, % Display a grid
%		%grid style={line width=.1pt, draw=gray!50}, % Set the style
%		xlabel={$ y $}, % Set the labels
%		ylabel={$ u $},
%		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%		x tick label style={rotate=0,anchor=north} % Display labels sideways
%		]
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/u_lcut_x_13.txt};
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/u_lcut_x_13.txt};
%		\legend{\tiny{$L_{FDM}$}, \tiny{$L_{FEM}$}}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		width=0.99\linewidth, % Scale the plot to \linewidth
%		%height=6cm,
%		%grid=major, % Display a grid
%		%grid style={line width=.1pt, draw=gray!50}, % Set the style
%		xlabel={$ x $}, % Set the labels
%		ylabel={$ u $},
%		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%		x tick label style={rotate=0,anchor=north} % Display labels sideways
%		]
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/u_lcut_x_33.txt};
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/u_lcut_x_33.txt};
%		\legend{\tiny{$L_{FDM}$}, \tiny{$L_{FEM}$}}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\begin{tikzpicture}
%		\begin{axis}[
%		width=0.99\linewidth, % Scale the plot to \linewidth
%		%height=6cm,
%		%grid=major, % Display a grid
%		%grid style={line width=.1pt, draw=gray!50}, % Set the style
%		xlabel={$ x $}, % Set the labels
%		ylabel={$ u $},
%		legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%		x tick label style={rotate=0,anchor=north} % Display labels sideways
%		]
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fdm/u_lcut_x_52.txt};
%		\addplot+ [thick, mark=none]
%		table[x expr={\thisrow{y}},y expr={\thisrow{u}},col sep=comma]{results_data/steady-heat-kl/sample-1/fem/u_lcut_x_52.txt};
%		\legend{\tiny{$L_{FDM}$}, \tiny{$L_{FEM}$}}
%		\end{axis}
%		\end{tikzpicture}
%	\end{minipage}
%	\caption{Dumb pictures of loss values}
%\end{figure}


%\begin{figure}[!htb]
%	\centering
%	%	\includegraphics[trim=100 0 619 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
%	\includegraphics[trim=0 0 0 0,clip,width=0.70\linewidth]{results_data/poisson-convergence/loss_all_annotated.png}
%	\caption{Loss plots for different resolutions}
%\end{figure}
% \subsubsection{Convergence studies}\label{sec:convergence-studies}
% To \ab{}


% \begin{figure}[!htb]
% \centering
% \begin{minipage}{.49\textwidth}
%   \centering
%  \begin{tikzpicture}
%      \begin{axis}[
%          width=0.99\linewidth, % Scale the plot to \linewidth
%          %grid=major, % Display a grid
%          %grid style={line width=.1pt, draw=gray!50}, % Set the style
%          xlabel= {\# step}, % Set the labels
%          ylabel=$\log_{10}(L)$,
%          legend style={at={(0.95,0.95)},anchor=north east,legend columns=1}, % Put the legend below the plot
%          x tick label style={rotate=0,anchor=north} % Display labels sideways
%       ]
%       \addplot [thick, mark=none]
%       table[x expr={\thisrow{Step}},y expr={ln(\thisrow{Value})/ln(10)},col sep=comma]{results_data/steady-heat-kl/loss_values.csv};
%      \end{axis}
%   \end{tikzpicture}
% \end{minipage}
%  \caption{Convergence of the error in $L^2$ norm for the Poissson equation with analytical solution $u =\sin{(\pi x)}\sin{(\pi y}$)}
% \end{figure}

%\subsubsection{In 2-D}
%4 terms in the K-L sum. 

% \begin{figure}[!htb]
% 	\centering
% 	%	\includegraphics[trim=652 0 100 0,clip,width=0.70\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_14.png}\\
% 	\includegraphics[trim={652 0 120 0},clip,width=0.98\linewidth]{results_data/run_003-fem-sobol-query/query_line_cut_15.png}
% 	\caption{Solution plot on horizontal line cuts at $y = 0.2, 0.5, 0.8$}
% 	\label{fig:poisson-kl-line-cuts-y}
% \end{figure}
\input{figure_panels/stochastic_histogram_panel.tex}
\subsubsection{Statistical distribution of solution}\label{sec:statistical-dist}
Since equation \ref{eq:poisson-kl-intro} is parametric, we can compare the quality of solution from \diffnet{} with a reference numerical solution in a statistical manner. We choose some points on the domain $ \spatialD $ (shown by markings on Fig. \ref{fig:query-points-for-statistics}) and evaluate the solution values at those query points for $ 20,000 $ samples of $ \diffusivity $. Therefore , at a particular query point, those $ 20,000 $ solution values approximately represent a distribution of the solution values at that point. So, we create a histogram of the solution values at each query point.
%\begin{figure}[!htb]
%	\centering
%	\includegraphics[trim=0 0 0 0,clip,width=0.35\linewidth]{results_data/run_003-fem-sobol-query/histogram_query_points.png}
%	\caption{Query points for histogram analysis}
%	\label{fig:query-points-for-statistics-0}
%\end{figure}


The histograms are shown in Figure~\ref{fig:stochastic-histograms}. We notice a very close match between the histograms obtained from \diffnet{} and a conventional FEM solver. This once again confirms that \diffnet{} is effective in providing the correct statistics of the parametric Poisson equation.


%\input{tables/sample-size-study.tex}

\subsubsection{3-D Poisson's equation}
So far, we have focused on two-dimensional problems. Although 2D problems are useful in demonstrating the key features and properties of \diffnet{} method, most of the real problems are three-dimensional. \ab{Please check the next statement} \diffnet{} can solve both 2D and 3D problems without much changes to the architecture. In Fig. \ref{fig:poisson-kl-3d-contours}, we show one randomly selected pair of $ \diffusivity $ and $ u $ for a 3D problem obtained using \diffnet{}.
\begin{figure*}[!htb]
	\centering
	\includegraphics[trim=90 0 800 400,clip,width=0.3\linewidth]{results_data/steady-heat-kl/nu_3d.png}
	\includegraphics[trim=90 0 700 400,clip,width=0.4\linewidth]{results_data/steady-heat-kl/nu_3d_sliced_view.png}
	\\
	\includegraphics[trim=90 0 800 400,clip,width=0.3\linewidth]{results_data/steady-heat-kl/u_3d.png}
	\includegraphics[trim=90 0 700 400,clip,width=0.4\linewidth]{results_data/steady-heat-kl/u_3d_sliced_view.png}
	\caption{Example of $\nu(x,y,z)$ and the solution $u^h_{\theta}(x,y,z)$ to the 3D Poisson's problem with log permeability}
	\label{fig:poisson-kl-3d-contours}
\end{figure*}



%\input{figure_panels/old_pyplot_histograms.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{(Possible exclusion) Steady reaction-diffusion equation}\label{sec:steady-reaction-diffusion}
% \begin{align}\label{eq:reaction-diffusion-steady}
% -\grad\cdot({\nu}(\mvec{x})\grad u) + \kappa^2 u &= f \text{  in  } D \\
% u|_{\partial \Omega} &= 0
% \end{align}
%
% The loss function:
% \begin{align}\label{def:loss-fem-reaction-diffusion}
% R = \int \left[{\nu}|\grad u|^2 + \kappa^2 u^2 - fu \right] d\mvec{x}
% \end{align}
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/reaction-diffusion/kappa-50/query_contour_0.png}
% 	\includegraphics[trim=100 0 70 0,clip,width=0.99\linewidth]{results_data/reaction-diffusion/kappa-100/query_contour_0.png}
% 	\caption{An example of solution of equation ~\ref{eq:reac-diff} for $\kappa = 50$ (top row) and $\kappa = 100$ (bottom row). From left to right: $f$, $u_{gen}$, $u_{num}$, $(u_{gen}-u_{num})$}
% \end{figure}
%
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[trim=140 0 645 0,clip,width=0.5\linewidth]{results_data/reaction-diffusion/kappa-50/query_line_cut_0.png}
% 	\caption{Solution plot on vertical line cuts at $x = 0.2, 0.5, 0.8$}
% \end{figure}
% \begin{figure}[!htb]
% 	\centering
% 	\includegraphics[trim=651 0 120 0,clip,width=0.5\linewidth]{results_data/reaction-diffusion/kappa-50/query_line_cut_0.png}
% 	\caption{Solution plot on horizontal line cuts at $y = 0.2, 0.5, 0.8$}
% \end{figure}

==> sections/temp-error-analysis.tex <==
Nothing
